Elastic Context: Encoding Elasticity for Data-driven Models of Textiles

Physical interaction with textiles, such as assistive dressing, relies on advanced dextreous capabilities. The underlying complexity in textile behavior when being pulled and stretched, is due to both the yarn material properties and the textile construction technique. Today, there are no commonly adopted and annotated datasets on which the various interaction or property identification methods are assessed. One important property that affects the interaction is material elasticity that results from both the yarn material and construction technique: these two are intertwined and, if not known a-priori, almost impossible to identify through sensing commonly available on robotic platforms. We introduce Elastic Context (EC), a concept that integrates various properties that affect elastic behavior, to enable a more effective physical interaction with textiles. The definition of EC relies on stress/strain curves commonly used in textile engineering, which we reformulated for robotic applications. We employ EC using Graph Neural Network (GNN) to learn generalized elastic behaviors of textiles. Furthermore, we explore the effect the dimension of the EC has on accurate force modeling of non-linear real-world elastic behaviors, highlighting the challenges of current robotic setups to sense textile properties.

==> includes/01_preliminaries.tex <==
%\section{Preliminaries and Related Work}
\section{Background and Related Work}
{\note old version}
\label{sec:preliminaries}


In this section, we review related work regarding the elasticity of textiles, their role in the robotic manipulation of deformable objects, and both analytic and data-driven approaches to encode such properties. Recent reviews provide an overview of flexible deformable objects and their use in dexterous robotic manipulation~\cite{hou2019review, yin2021modeling}.


\subsection{Elasticity in Textiles}
Physical properties of textile objects like elasticity, surface friction, and flexibility are mostly determined by the yarn material and the construction or production technique of the textile~\cite{grishanov2011structure}. Common yarn materials are, for example, cotton, wool, or polyester. In modern textiles, these raw materials are blended with elastomers, such as elastane, making the yarn intrinsically more flexible and widening the range of possible elastic behaviors exhibited by textile samples~\cite{uyanik2019strength}. The construction technique, which is usually woven or knitted, determines how the yarn threads are interlaced or interloped. Woven textiles, such as jeans, are produced with two sets of tightly interlaced yarns that make the textile rather rigid. Knitted textiles, on the other hand, are made with one interloped thread. This construction technique makes the loops in the textile generate open spaces between parallel running threads, resulting in more stretchable textiles than woven ones. For a more detailed description of different construction techniques, we refer to the recent textile taxonomy in~\cite{longhini2021textile}. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/breakpoint.png}
    \caption{Typical stress curve for manipulation of elastic textiles: in the \emph{free} manipulation phase, no forces are exerted on the robot end-effectors; in the \emph{stress} manipulation phase, the properties of the textile (such as the elasticity) determines its behavior and the forces sensed; finally, if the force applied is too large, the textile breaks.}
    \label{fig:phases}
\end{figure} 

The evaluation of the elastic behavior of textiles is usually done with the Stress-Strain test, where a fixed load is applied to a piece of textile, and the percentage of displacement, also called strain, is measured~\cite{kawabata1989fabric, eberhardt1996fast}. 
Prior work~\cite{longhini2021textile} used the end-effector of a robot to generate different force loads on the textile, resulting in textile-specific profiles that can be decomposed into the three-different stages shown in Fig.~\ref{fig:phases}. In the first stage (\textit{free} manipulation), no stress is introduced by the end-effector as the deformable nature of the textile makes it compliant with the robot's movement. In the second phase (\textit{stress} manipulation), the textile starts to induce forces on the end-effector, and its mechanical properties, such as elasticity, become important to consider. Finally, after a certain textile-specific force, the textile reaches a breaking point. Often in robotic tasks, objects are manipulated within the \textit{free} manipulation phase. 
Nevertheless, precise modeling of the \textit{stress} manipulation phase can be useful for applications requiring a constraint over the forces exerted on the deformable object or to assure that a specific action is performed correctly~\cite{erickson2018deep,chi2022iterative}. These tasks have been addressed so far with the implicit assumption that the elasticity of different manipulated samples do not exhibit large variations in their dynamics, despite the wide diversity of real-world elastic textiles (such as first-aid bandages, t-shirts, jeans). In this work, we consider the learning of models of textile samples capable to generalize to different and unseen elastic behaviors by leveraging our proposed \emph(Elastic Context).



\subsection{Analytical Models of Elasticity in Textiles}

Analytical models of textiles usually rely on physics-based modeling and geometric representations, such as particles or meshes~\cite{yin2021modeling}. 
\acp{pbd} approaches model the displacements of a discrete system of particles by applying geometrical constraints~\cite{arriola2020modeling}. This strategy is computationally efficient but struggles to model net forces and is resolution dependent~\cite{eberhardt1996fast}. Mesh models overcome these problems by encoding the interaction between the particles in the edges of the mesh. In mass-spring models, the edges represent springs following Hooke's law to encode linear elastic relationship \cite{wang2011data}. Damping, bending, and shearing factors can be integrated to reproduce more complex behaviors. However, linear approximations of the textile dynamics underperform with large deformations. The high strain regime cannot be ignored when modeling textiles as such deformations may occur near the garment’s seams or when parts of the textile are physically constrained. Non-linear models, such as the Neo Hookean or the St. Venant–Kirchhoff, have the advantage of being more accurate than the mass-spring models, but their computational complexity is not suitable for real-time simulations~\cite{boonvisut2012estimation,clyde2017modeling, miguel2016modeling}.
%To deal with large displacements, more complex constitutive approaches such as the Neo Hookean or the St. Venant–Kirchhoff models are used to encode non linear hyperelastic relations \cite{boonvisut2012estimation,clyde2017modeling, miguel2016modeling}.  These models have the advantage of being more realistic than the mass-spring models, but their computational complexity is not suitable for fast simulations. 
In robotic manipulation tasks, task-specific and low-dimensional textile representations are often favored over a precise description of all possible mechanical behaviors of the textiles~\cite{mcconachie2020interleaving}. Finding a suitable trade-off between the model accuracy and numerical efficiency is therefore of fundamental importance~\cite{marinkovic2019survey}.


\subsection{Data-driven Models of Textiles}
A limitation of analytical models is the requirement of having precise knowledge of the physical parameters of the textile, which hinders their application in real-world scenarios, where the properties of deformable objects are often unknown. Despite the effort to simplify the complex measurement tools used in textile engineering, the estimation of textile parameters remains highly engineered~\cite{wang2011data, miguel2012data}. Black-box models like neural networks provide a viable solution to model dynamic behavior without explicit knowledge of all the parameters. \acp{gnn} have shown to be a particularly powerful framework in the context of learning mesh-based dynamics, being employed in a variety of complex domains, including deformable objects~\cite{georgousis2021graph, chang2016compositional, lin2022learning}. 
Battaglia,~\etal~\cite{battaglia2016interaction} proposed Interaction Networks (INs) to learn a physical engine to capture local interactions among nodes by modeling them through a complete graph. Li ~\etal~\cite{li2019propagation} extended this framework by proposing Propagation Networks (PNs), which enable instantaneous propagation of forces by multi-step message passing. These approaches have shown excellent results in modeling deformable objects, but they assume the parameters of the object are known a priori. In this work we relax this assumption by suggesting to leverage a large variety of elastic behaviors, conditioning a GNN on our proposed \emph{Elastic Context}. 


==> includes/03_RW_SIM.tex <==
\section{Sim-Real Gap}
\label{sec:realVSsim}
%\section{The Real World and Simulation}

\begin{figure*}[!t]
   \centering
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{images/bullet_profiles.png}
         \caption{Simulated profiles}
         \label{fig:bullet_profiles}
     \end{subfigure}
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{images/real_profiles.png}
         \caption{Real-world profiles}
         \label{fig:rw_profiles}
     \end{subfigure}
    \label{fig:force_profiles}
    \vspace{-0.2cm}
    \caption{{\red missing the correct labels, teh idea is to categorize the with the same strategy that real world fabrics are cathegorized, by placing the percentage of elongation. }}
\end{figure*}

% {\color{teal}

% \begin{itemize}
%     \item The data-driven models described in the previous section will learn the behavior contained in the training data.
%     \item Here we analyse what real-world and simulated behaviors look like.
%     \item For simulated behavior we consider the following models: ideal mass-spring model and  mass-spring damper model of Bullet.
%     \item Analysis of the cool figure and some comments about the discrepancies.
% \end{itemize}

% % PROS AND CONS not anymore

% % The choice between one of them is highly dependent on the task that has to be solved by the robot. Put a TABLE to describe the main concepts of pros and cons and briefly discuss them.

% % \begin{itemize}
% %     \item comparison between manipulation task execution
% %     \item comparison between access to ground truth meshes and Force Feedbacks
% %     \item comparison between the variety of the underlying models that can be learned {\color{red} Most of this is not news to any one in robotics? we should focus specificly on the modeling of deformable objects with it's new focus from the comunity.}
% % \end{itemize}

% }
{\red Shorten this part...}\\
When employing data driven models, the quality and amount of the training data is of utmost importance for the performance of the model. As collecting real world data is often time and cost intensive, a common approach is to leverage data collected in simulation. A common prerequisite for simulators used in robotic computational efficiency to allow real time perception and manipulation. To meet this requirement, model accuracy 
%However, in order to bridge the Sim-to-Real gap, modeling the real world system as accurately as possible is crucial. When modeling complex systems or phenomena, a trade-off must be struck between accuracy and computational efficiency {\color{red} CITE HANG SURVAY?}.
%If the simulator also has to facilitate many different domains, i.e: rigid- and deformable objects, measuring interaction forces between them and kinematic actors, the constrain becomes more difficult to fulfill. {\color{red} MW: mmmm not that happy with this formulation ...}
 However, there is a sim-to-real gap and it is ideal to reduce the reality gap in order to more effectively transfer learned knowledge to the real world
In this section we take a closer look into the differences between the real world elastic behavior of fabrics and commonly used simulation approaches from the robotic domain.

%A common approach to model cloth like objects is by modeling it as a 2D grid of nodes with constrains between the nodes, this constrains are often modeled as springs, or spring-dampers. This resulting in so called mass-spring models that are used to model cloth in the commonly used Bullet physics engine {\color{red} CITE} and the popular reinforcement learning simulator Mujoco{\color{red} CITE} (Mujoco refers to constrains between the 2D nodes as tendons) {\color{red} MW: I'm a bit out of my depth here so we might want to hedge certain thinks or separately validate them.}

In order to simulate different elastic behaviors a number of parameters can then be set in order to achieve the desired results. In the case of a simple mass spring model that is solely based on Hook's Law only the spring constant can be altered, while Bullet for example offers three parameters in order to influence the behavior, namely spring - \textit{elastic}, \textit{damping} and \textit{bending} - stiffness.
Choosing the correct parameters is nontrivial and the resulting effects are hard to predict and can sometimes even result in unstable simulation of the fabric. {\color{red} MW: It's mostly users that don't have many experience with it I would say ...}



% {\al

% Data driven methods offer the opportunity to describe objects behaviors without knowing a priori the underlying analytical model and the corresponding parameters. However, they have the drawback of being limited to learn the implicit pattern contained in the data used to train them. In what follow, we will therefore evaluate different fabric models used in robotics, spanning from an ideal scenario to real-world behavior.\\
% To gather meshes and force feedback needed to describe elastic fabrics and train black-box models there are two viable approaches. The first one rely on simulators capable to model deformable objects and their relative force responses. In this analysis we chose to use the Bullet engine {\red cite} as it is among the most used ones  for robotics applications and fits our requirement of providing force feedback in PyBullet. This physics engine can use either Position Based Dynamics (PDB) model or the mass-spring-damper one. For stability reasons, we focused on the latter {\red maybe few sentences might be fixed/rewritten by Zackory}. \\
% The alternative to simulators is to collect measurements from the real world through interaction with different fabrics. In this circumstance,  precise analytical model cannot be defined. The observed behaviors depend on the underlying fabric properties   such as material and construction technique described in section \ref{sec:preliminaries}. \\
% In what follow, we will discuss how the data collected with these two methods exhibit different behaviors of fabric. In particular we will focus on the evaluation of the stress/strain response of different elastic textiles, leaving the analysis of other mechanical properties such as surface friction or breaking force for future work. Moreover, we extend the comparison by including in the discussion data collected form a simulated ideal mass-spring model.\\ }

To get a good overview of how accurate current simulator such as bullet approximate the real world we perform the Stress-Strain test discussed in section {\color{red} REF}.
We collect the force-displacement profiles from {\color{red} XX} real world samples with different elasticity's by pulling them with two robotic grippers equipped with force/torque sensors until a maximum force of $7.7 $ N is reached. We perform the same test in pybullet where we vary the \textit{elastic}, \textit{damping} and \textit{bending} parameters until a force of {\color{red} XX} is recorded. 
{\color{red} ALEX SIMULATOR}
The real world Stress-Strain curves are show in Fig. {\color{red} REF} left while the bullet once are shown on the right. Note that we assume the cloth to be at the beginning of \textit{manipulation phase 2} as indicated by Fig. {\color{red} REF} where the fabric is stretched but not under stress.

We can see that the real world follow the three phases highlighted in Fig. {\color{red} REF}:
An initial phase of initial resistance to deformation, a region of low deformation, and a final region of high deformation {\color{red} MW: wait, the final region is NOT high deformation!!! we need to check this} before the breaking point \cite{breen1994predicting}.
{\red change the analysis of the phases, we don't have them anymore}
The bullet simulation models successfully the first two deformation phases thanks to the included damping factor in it's model, but fails to account for the nonlinear region at the end.
Furthermore, we did not manage to model a similar diversity of elasticity in simulation as in the real world without the simulator becoming unstable.

We can summarise our observations, that while the simulation model can accurately imitate the initial and linear behavior it does not model the finale non linear phase observed on the real fabric. {\color{red} IMPLICATIONS OF THIS in 2 or 4 sentences.}



% {\al
% % Discussion about the final figure
% \subsection{Stress-Strain Comparison}
% {\red Missing a specificaiton about the range of displacement for each model: real-world is limited by robot's constraints, while simulation could potentially go on forever.}
% The stress-strain curves of fabrics could be divided in three regions: region of initial resistance to deformation, a region of low deformation, and a region of high deformation \cite{breen1994predicting}.  In the low deformation region the assumption of linear elasticity yield reasonable cloth-like behaviors. The same does not hold for the initial-resistance and high deformation regions. Therefore, the mechanical behavior of the cloth throughout its range of deformation is  non-linear, especially during the initial/high deformation regions.\\
% Figure \ref{fig:force_profiles} shows the force profile collected in the three different scenario introduced above. Comparing the ideal mass-spring model (right) with Bullet's model (middle), it can be concluded that the addition of the damping factor on Bullet allows to correctly model the initial non linearity. Bullet, however, struggles to describe high-deformation regions as it exhibits a linear behavior for the rest of its profile. Worth to be mentioned is that fabrics are assumed to be infinitely stretchable due to the complexity of modeling their breaking point {\red can be written better or even removed}.
% Moving to the analysis of the real world force data (left), it can be seen that textiles show complex and diversified stress-strain trends. More rigid samples exhibit a behavior close to the simulated one as they reach fastly the maximum strength that the robot can apply during the movement. For what concern the more elastic samples, it is easier to observe the two non-linear regions aforementioned as their maximum displacement is further than the rigid ones. This allows to observe high strain regions. Lastly, it is interesting to notice how it is also possible to observe quasi-linear behaviors when constraining the displacement to the robot work space.\\
% % It can be seen from the left image that the real-world exhibits a wide range of behaviors, from non-linear to almost linear ones.
% It can be concluded that analytical model used to model fabrics in robotic simulators are not as expressive as the real world in therms of elastic behaviors. For practical reasons, simulators trade off accuracy against computational efficiency. This leads them to be less suited for learning data-driven models due to the real-simulation gap of the elastic model of fabrics. {\red can be written better}


% % Here conclude by mentioning the diversity of the real world with respect to the analytical models.
% %in the middle, exploits the initial non-linear behavior, therefore it's closer to the real world with respect to the ideal mass-spring model showed on the right. However, the behaviors it can model it no as divers as the real one.  {\red what else can be said about the figure?} \\

% {\red What follow is not finished. Use this in the conclusion, not here...}
% It can be concluded that fabrics models used in robotic simulator still not close enough to the real-world, moreover elasticity is not the only property that cannot be properly modeled. Other complex effects such as surface friction, slipping and breaking point of the garment are challenged to be integrated due to the complexity of the analytical model. Another limitation is the challenge to include perception in simulators such as F/T measurements. However these things are important for robotic tasks such as....
% The drawback of real world data is the complexity of the data collection. Ground truth meshes are difficult to obtain due to self occlusions. Complex manipulation strategies are as well complex. There might be the chance to do real to sim....

% }



==> includes/04_related_work.tex <==
\section{Related work}



\subsection{Learning Textile Representations}
Graph neural networks have shown to be a particularly powerful framework in the context of learning mesh-based dynamics, being employed in a variety of complex domains \cite{georgousis2021graph, chang2016compositional}. 
Battaglia,~\etal~\cite{battaglia2016interaction} proposed Interaction Networks (INs) to learn a physical engine to capture the underlying physical interactions by modeling them as a complete graph over the particles. This model can then be used to predict future states of the object. However, INs cannot handle propagation of forces as they consider just local information. To overcome this problem \cite{li2019propagation} proposed propagation networks (PNs) which enable instantaneous propagation of forces by multi-step message passing. 
In a previous work, \cite{li2018learning} used GNNs to learn particle-based  dynamics by using a graph that dynamically changes through time instead of being static, allowing the model to approximate more complex dynamics and interactions involving discontinuous functions (e.g. contact). Moreover, they introduced a hierarchy to deal with long-range dependencies. \cite{pfaff2020learning} learned a mesh-based simulator with GNNs, where they adopt an adaptive re-meshing algorithm to increase the scale of the representation when needed. This method, differently from the ones previously mentioned, considered textiles as deformable objects and showed good results in modeling clothes behaviors.
{\red Missing conclusion where we specify what we do differently}

\subsection{Robotic Manipulation of Textiles}
% In robotic manipulation tasks, task-specific and reliable textile representations are often favoured over a precise description of all possible mechanical behaviors of the fabrics. Many approaches opt to represent only task relevant features of the deformable object, employing simplified models {\color{red} CITE BERENSON ROPE?}, or focus on tasks where modelling elastic aspects are of limited importance such as grasping, folding or flattening {\red cite maybe a review of tasks}. 
For tasks such as assistive dressing, modelling elastic properties can be advantageous to predict when too much force is exerted on the person dressed or to assure that a specific dressing action is being performed correctly {\color{red} CITE}. These tasks have been addressed so far with the implicit assumption that the elasticity of different manipulated samples does not significantly change, despite the wide diversity of potential fabrics suitable to be employed in assistive dressing tasks, such as first-aid bandages, t-shirts, jeans. In this work, we consider the learning of models of textile samples with elastic context, allowing for generalized representations of the behavior of these objects suitable for robotic manipulation.

\begin{comment}
{\color{teal} 
The main topics that have to be discussed in this section are:
\begin{itemize}
    \item learning mesh models of fabrics : simulation and real-world cases
    \item elastic parameter identification
    \item differences between real-world and simulation behaviors.
\end{itemize}



}
Graph neural networks have shown to be a particularly powerful framework in the context of learning mesh-based dynamics, being employed in a variety of complex domains \cite{georgousis2021graph, chang2016compositional}. 
\cite{battaglia2016interaction} proposed Interaction Networks (INs) to learn a physical engine to capture the underlying physical interactions by modeling them as a complete graph over the particles. This model can then be used to predict future states of the object. However, INs cannot handle propagation of forces as they consider just local information. To overcome this problem \cite{li2019propagation} proposed propagation networks (PNs) which enables instantaneous propagation of forces by multiple message passing. 
In a previous work, \cite{li2018learning} used GNNs to learn particle-based  dynamics by using a graph that dynamically changes through time instead of being static, that allows the model to approximate more complex dynamics and interactions involving discontinuous functions (e.g. contact). Moreover, they introduce hierarchy to deal with long-range dependencies. \cite{pfaff2020learning} learned a mesh-based simulator with GNNs, where they adopt an adaptive remeshing algorithm to increase the scale of the representation when needed. This method, differently from the ones previously mentioned, considered textiles as deformable objects and showed good results in modeling clothes behaviors.
{\red missing what we're doing different from them}
{\red add the paper that are learning models from real world but that are not elastic}
{\red add the papers that evaluate mismatches between real and simulation}

\end{comment}







==> includes/05_dataset.tex <==
\section{Experimental Evaluation }
% {\color{teal}

% \begin{itemize}
%     \item task decscription
%     \item generation details of simulated dataset
%     \item generation details of real-world dataset
% \end{itemize}


% }

% {\color{teal}
% \begin{itemize}
%     \item Overview
% \end{itemize}
% }
% introduction of the task

\begin{comment}




{\red still to verbose, needs to be shortened}
In this section we present the experimental evaluation to assess the performance of the proposed \emph{Elastic Context} introduced in section \ref{sec:method}.  To this end, we devised a simplified assistive dressing scenario, where a dual arm robot is asked to stretch a piece of fabric over a sphere resembling the head of a person.  Each different execution is performed using a different sample with a different elasticity, to exhibit the different elastic behaviors of fabrics introduced in section \ref{sec:realVSsim}.  The data obtained from this task is then used to train our proposed model to perform a \textit{force forecasting} task, which consists of predicting multiple steps in the future starting form the moment of the contact with the object in order to observe the force profile specific for any elastic sample.
With this scenario, the goal is two-fold, to highlight the relevance of the elastic context and to show the capability of our model to reason about two physical concepts: the future state of the fabric (approximated as a graph) and the evolution of the forces recorded at the end-effectors.  


%We compare our proposed models with models that do not have access to the elastic context information discussed in section \ref{sec:method}.
%While we assume access to force readings in order to obtain the context. No such assumption is made for the bandaging task itself. The context also does not need to be obtained with the robot performing the manipulation but could for example be acquired by {\color{red} EXAMPLE}.
\noindent
\textbf{Task set-up:} To collect the sequences of meshes with the relative force perceived, we reproduced the aforementioned scenario both in real-world and simulation.
An overview of the setup can be seen in Fig.\ref{fig:envronments}, where two robotic grippers either pull a piece of fabric or stretch it over a rigid sphere. To manipulate the fabric in the real-world setting (right) we used two Franka-Emika Panda equipped with Optoforce Force/Torque sensors {\red cite}, while in simulation (left) we replicated just their end-effectors as "floating" grippers and their force perceived.

%In the simulation (left) two floating grippers are holding a piece of fabric between them being able to move in the indicated Y- and Z-Axis, in order to pull the fabric over the white sphere. On the right the real world setup is shown where two Franka Panda robots are holding a piece of fabric between them, ready to pull the fabric (X-axis) and stretch it over the 3D-printed head model. 

\begin{figure}[h!]
  \centering
  \includegraphics[width=1\linewidth]{images/pull&task}
  \caption{Real world (left) and simulation (right) environments. The  \textit{y} axis corresponds to the pulling direction used to collect the context, while the \textit{z} axis is related to the task execution. }
  \label{fig:envronments}
\end{figure}


%\subsection{Implementation detail}
\noindent
\textbf{Data-Collection:} The ground truth forces are recorded from the force sensors on the writs of the robot grippers both in real world and simulation. The position of the grippers allowed us to compute the stretch of the cloth. For what concerns the graph representations, the simulation provides the ground truth positions for all cloth vertices disposed as  a $25\times25$  3D mesh that we downsampled to $12\times12$ for computational reasons. To obtain the same data in the real world, we placed 25 markers in a $5\times5$ grid in the manipulated textile,  and we extracted its 2D vertices from images recorded with an RGB camera mounted above.
% Context collection
The first stage of the task is the collection of the elastic context, which is obtained by moving the grippers in opposite directions along the Z-axis and stretching the cloth up to a force perceived of $7 N$. The displacement-percentage is then computed following the context definition provided in Sec. \ref{sec:method}.
% Initialization and execution of the task
The second phase is the execution of the task, where the robots pull the cloth over a sphere for $15cm $ or util he perceive a force threshold of $7 N$. The grippers are initialized assuming that the starting position of the cloth is such that it is stretched with minimal force, (beginning of phase 2 in Fig. {\color{red} REF TODO}. 


\noindent
\textbf{Elastic samples:}
%The data collected consist of {\color{red} XX}, and {\color{red} XX} task repetitions for the simulated and real world setting respectively.
Each task repetition was executed varying the intrinsic properties among different fabrics in order to observe diverse elastic behaviors.
For the simulation we selected the \textit{elastic} parameter in the interval $[14,39]$, sampling with a step of 5 and the \textit{bending} parameter in the interval $[7, 14]$ with a step of 1. We fixed the \textit{damping} to $0.5$ as different values were generating unstable meshes. These intervals have been chosen based on simulation limits. {\color{red} (write better in the sense that simulation explodes)}. {\red for the real world data we should find  way to describe their elasticity, we might use the same method of Spain...}

\noindent
\textbf{Training details:} For the evaluation of the \textit{context}, we employed our proposed GNN model, as well as a standard MLP architecture {\red cite}, which allow us to understand the influence of the \textit{context} in the \textit{force forecasting} also when the model is not required to predict the dynamics of the mesh. The baseline version of these models receive as input the initial position of the grippers and the action to be performed, defined as relative displacement, while the conditioned models that we propose have access to the elastic context as well. The output for the MLP is the prediction of the force perceived if the robot performs the input action, while for the GNN it is the combination of the force and mesh predictions. To make the comparison as fair as possible the same core architecture is used for all models, composed of six linear layers {\red propagation steps missing}. The graph prediction and force prediction head consist of one linear layer and two linear layers respectively. All linear layers have 16 hidden units, and in between the ones not involved on the propagation step of the GNN, we used Rectified Linear units (ReLu) as activation function.
We train all models for $1000$ epochs, set mini batch size to 32, the learning rate to $0.0003$, and a test/train split of $0.2$. The parameters were optimized using Adam {\red cite}. All the training objectives and test measures for the forces used mean squared error (MSE) between the model's prediction and the ground truth. For what concern the graph, we used the sum of the squared euclidean distances computed at each node between the predicted ones and the ground truth. 







\begin{comment}

\subsection{Comparison and evaluation Criteria}
We compare four different models agings, two models making use of the elastic context and two baseline models. In detail this models are:
\emph{i)} \textit{GNN-B}, a GNN based model without access to the context.
\emph{ii)} \textit{GNN-C}, a GNN based model with acces to the context.
\emph{iii)} \textit{MLP-B}, a MLP based model without acces to the context.
\emph{iv)} \textit{MLP-C}, a MLP based model with acces to the context.



\subsection{Prediction Results}
We compare our proposed models with models that do not have access to the elastic context information discussed in section \ref{sec:method}.
{\color{red} TODO Simulation Results, + discussion thereof}

The results of the real world bandaging task for the force prediction are shown in Fig. {\color{red} REF}. We can make two core observations: \emph{i} Models that make use of the elastic context achieve significant lower prediction error than models that do not use the context. Highlighting the importance of giving context to predictive models.
\emph{ii)} GNN based models converge faster then MLP based models. We hypothesise that the faster convergence is due to the inductive bias imposed by the GNN by using a propagation model, as both the graph and force dynamic are dependent on the interaction between fabric nodes and a GNN naturally exploits this relationships as pointed out in \cite{li2019propagation}

    \begin{figure*}[!t]
         \centering
         \begin{subfigure}[b]{0.4\textwidth}
             \centering
             \includegraphics[width=\linewidth]{images/2D_sim.png}
             \caption{SIMULATIOIN.}
             \label{fig:force_context_loss}
         \end{subfigure}
         \begin{subfigure}[b]{0.4\textwidth}
             \centering
             \includegraphics[width=\linewidth]{images/force_context_loss.png}
             \caption{REAL WORLD}
             \label{fig:graph_context_loss}
         \end{subfigure}
    \label{fig:test_losses}
    \end{figure*}
    


\subsection{Raw Results - Force prediction}





\begin{table}[!h]
\centering
\caption {MLP - Simulation 3D (smoothed 0.9)}
\begin{tabular}{|l|l|}
\hline
        &  \textbf{Min loss value $[N * 10^{-3}]$}   \\ \hline
% long sleeve top     &  4 steps - 80\%                                        \\ \hline
baseline     &          8.34                        \\ \hline
Context size 2    &      \textbf{7.39}                              \\ \hline
Context size 10           &      8.21                           \\ \hline
\end{tabular}
\label{tab:manipulation_results}
\end{table}

\begin{table}[!h]
\centering
\caption {GNN - Simulation 3D (smoothed 0.9)}
\begin{tabular}{|l|l|}
\hline
        &  \textbf{Min loss value $[N * 10^{-3}]$}   \\ \hline
% long sleeve top     &  4 steps - 80\%                                        \\ \hline
baseline     &          8.77                        \\ \hline
Context size 2    &         \textbf{7.91}                          \\ \hline
Context size 10           &           8.17                      \\ \hline
\end{tabular}
\label{tab:manipulation_results}
\end{table}


\begin{table}[!h]
\centering
\caption {MLP - Simulation 2D (smoothed 0.9)}
\begin{tabular}{|l|l|}
\hline
        &  \textbf{Min loss value $[N * 10^{-3}]$}   \\ \hline
% long sleeve top     &  4 steps - 80\%                                        \\ \hline
baseline     &            8.34                      \\ \hline
Context size 2    &            \textbf{7.50}                     \\ \hline
Context size 10           &           8.18                      \\ \hline
\end{tabular}
\label{tab:manipulation_results}
\end{table}


\begin{table}[!h]
\centering
\caption {GNN - Simulation 2D (smoothed 0.9)}
\begin{tabular}{|l|l|}
\hline
        &  \textbf{Min loss value $[N * 10^{-3}]$}   \\ \hline
% long sleeve top     &  4 steps - 80\%                                        \\ \hline
baseline     &             8.67                     \\ \hline
Context size 2    &       non pervenuto       (edges 8.77)                     \\ \hline
Context size 10           &    \textbf{8.27} (early stopping) (edges 8.18)                         \\ \hline
\end{tabular}
\label{tab:manipulation_results}
\end{table}



\begin{table}[!h]
\centering
\caption {MLP - Real-world 2D (smoothed 0.9)}
\begin{tabular}{|l|l|}
\hline
        &  \textbf{Min loss value }   \\ \hline
% long sleeve top     &  4 steps - 80\%                                        \\ \hline
baseline     &         0.49                         \\ \hline
Context size 2    &           0.253                         \\ \hline
Context size 10           &           \textbf{0.198}                      \\ \hline
\end{tabular}
\label{tab:manipulation_results}
\end{table}


\begin{table}[!h]
\centering
\caption {GNN - Real-world 2D (smoothed 0.9)}
\begin{tabular}{|l|l|}
\hline
        &  \textbf{Min loss value }   \\ \hline
% long sleeve top     &  4 steps - 80\%                                        \\ \hline
baseline     &               0.55                   \\ \hline
Context size 2    &              \textbf{0.18}                     \\ \hline
Context size 10           &           \textbf{0.185}                      \\ \hline
\end{tabular}
\label{tab:manipulation_results}
\end{table}




\end{comment}


\subsection{Context Evaluation}
{\red I would replace these results with the one obtained from the GNN, using a table to insert the the comparison of the perfomances between the force prediction of the MLP and the GNN}
We chose to showcase the role of the context  in the simulation scenario, as it was possible to precisely tune the ground truth parameters of the underlying model of the textile.  We evaluated the performance of the baseline and conditioned MLP architectures on the \textit{force forecasting} task. Moreover, to understand the effect of the size  the role of the size of EC ($n_c$) we downsampled the original context profile as described in Section~\ref{sec:method}. We present the force-profiles obtained in Fig.~\ref{fig:mlp_context}. The results show that only the models with EC are able to generalize their force predictions to unknown samples. As shown in Fig.~\ref{fig:no_context}, without EC, the force prediction collapses, predicting the same profile regardless of the samples. This highlights the fundamental nature of considering EC to generalize force-predictions to unseen samples. Employing a smaller EC ($n_c = 3$) widens the range of predictions of the model, yet, as seen in Fig. \ref{fig:context_3}, it still struggles to cover the spectrum of all possible test profiles. The performance of the prediction models improves with increasing EC size, as shown in Figures \ref{fig:context_40} and \ref{fig:context_80}. However, the increased  EC with $n_c = 80$ does not significantly improve the quality of the model's prediction, as shown in Fig.~\ref{fig:context_80} despite the increased computational overhead.

%The experiments aims to show:
%\begin{itemize}
%    \item The relevance of the context to distinguish the force response of %different elastic samples
%    \item The effect of the size of the context on the force prediction
%\end{itemize}


\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.49\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{images/prediction_mlp.png}
         \caption{Baseline MLP $(n_c = 0)$}
         \label{fig:no_context}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{images/prediction_mlp_c3.png}
         \caption{MLP + EC $(n_c = 3)$}
         \label{fig:context_3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{images/prediction_mlp_c40.png}
         \caption{MLP + EC $(n_c = 40)$}
         \label{fig:context_40}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.49\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{images/prediction_mlp_c80.png}
         \caption{MLP + EC $(n_c = 80)$}
         \label{fig:context_80}
     \end{subfigure}
\caption{Force-forecasting of dynamics prediction models with different number of steps $n_c$ of EC in unseen elastic samples. We show the ground-truth force-profiles (in blue) and the predicted force-profiles (in red) of test samples. The results show that the dynamical prediction models are only able to accurately generalize to unseen textiles with EC. Best viewed with zoom.}
\label{fig:mlp_context}
\end{figure*}

%The test results of the force profile predictions for each different model are presented in Fig. \ref{fig:mlp_context} . It can be seen how the model without the elastic information (Fig. \ref{fig:no_context}) always predicts the same profile for different samples. Using a context of size $3$ (Fig. \ref{fig:context_3}) slightly widen the range of prediction of the model, but it still struggles to cover the spectrum of the test profiles. Figures \ref{fig:context_40} and \ref{fig:context_80} highlight two facts: a bigger context helps to improve the quality of the model's prediction, but a  larger contexts does not necessarily contain more information.


\subsection{Elastic Mesh Models}
{\red should we add quantitative results?}
We evaluate the performance of the GNN-based representation with EC in predicting the position of the nodes in unseen textile-graphs. We show graph-predictions both in simulation (3D) and in real-world (2D)  settings in Fig.~\ref{fig:GNN_mesh_predt}. The results show that GNN with EC is able to accurately predict the future prediction of the position of the nodes of unseen textile-meshes, both in simulation and in real-world settings

%We evaluate the performance of the GNN-based representation with EC in predicting the position of the nodes in unseen textile-graphs. We perform a rollout of 10 steps starting from the initial state prediction for the mesh in simulation (3D) and in real-world (2D) and visualize the results in Figure \ref{fig:GNN_mesh_pred}, where we can see how the GNN can learn the dynamics of the task and reproduce it in a rollout efficiently. 

\begin{comment}
%We provide the quantitative results of the prediction error in Table \ref{tab:GNN_dynamic_mesh_comparison} {\color{orange} context beats baseline gnn?}.


\begin{table}[!h]
    \centering
    \begin{tabular}{ccccc}\toprule
         & \multicolumn{2}{c}{MLP} & \multicolumn{2}{c}{GNN } \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
          Env.          & no C & C  & no C & C  \\ \midrule
         RW     &  - &- &-  & - \\
         SIM     &  0.0913 & 0.0561 & - &  0.0503 \\ \bottomrule
    \end{tabular}
    \caption{Graph prediction error rollout 10. Effect of the types of conditioning and on the modelling of the force dynamics.}
    \label{tab:GNN_dynamic_force_comparison}
\end{table}

\end{comment}


\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.9\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{images/RW_mesh_prediction2.png}
         \caption{2D mesh predicted by the GNN in real world {\red to be changed}}
         \label{fig:GNN_force_pred}
     \end{subfigure}
     \begin{subfigure}[b]{0.9\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{images/mesh_prediction.png}
         \caption{3D mesh predicted by the GNN in simulation}
         \label{fig:GNN_mesh_pred}
     \end{subfigure}
\caption{Graph predictions of the GNN model with ~\emph{Elastic Context}. We show the original graph (in grey) along the predicted (in red) and the ground-truth (in blue) graphs after 10 steps. }
\label{fig:mesh_predictions}
\end{figure}

\subsection{Sim2Real Gap}
{\red missing any kind of discussion about simulators}
To conclude our evaluation, we chose to present an experiment that displays the gap between real and simulated elastic behaviors.
{\red missing a brief description of figures \ref{fig:bullet_profiles, fig:force_profiles}}
For this evaluation we selected the conditioned MLPs trained simulation, and tested its capabilities to transfer the knowledge into the real-world domain.
%, real world exhibits elastic behaviors that are more chaotic with respect to the ones observed in simulation. To provide an insight on the consequences of this gap, we used the real-world dataset to train the same model architecture as the simulation one using a context of dimension {\red X}. We therefore tested the transfer capabilities of both real and simulated model to the opposite domain. 



Fig.~\ref{fig:sim2real} highlights how the MLP model trained on the simulated data fails to adapt its predictions to the real-world data. To understand such results and the accuracy of the employed simulator we present a random subset of profiles from both simulated and real-world data, show in Fig.~\ref{fig:bullet_profiles, fig:force_profiles}. We observe significant differences between the data collected in both scenarios. In particular, the simulation profiles fail to account for the nonlinear behaviour at the end of the real-world profiles. Furthermore, despite extensive hyperparameter searching, we did not manage to model a similar diversity of elasticity in simulation as in the real world data without the simulator becoming unstable.

Thus, while the simulation model can accurately imitate the initial and linear behavior of the real-world data, it fails to model the final non-linear behavior observed on real fabric. This observation motivates the need for the development of improved simulation environments that are able to capture the rich behavior of real-world highly-deformable objects (such as textiles) for sim2real manipulation tasks.

\end{comment}


\begin{comment}

{\al
% Task description
The goal of the robotic task is to show the capability of our model to reason about two physical concepts: the future state of the manipulated cloth and the force feedback perceived along the task. While the the state prediction could be generalize to different fabrics, the same does not hold for the force feedback due to different elastics responses that fabrics might have. Our proposal to overcome this challenge, is to make use of an elastic context that can be easily collected by the robot ahead the task execution.  
In order to evaluate the relevance of the elastic context on force prediction, we devised a simplified assistive dressing scenario. The goal is to reproduce the case where the garment gets stuck while dressing someone, to exhibit the different elastic behaviors of distinct fabric samples. To achieve this target, a dual arm robot is asked to perform a two-stage pipeline while manipulating a rectangular textile with no holes. The two stages consist in: pull the object to collect the elastic context, drag {\red ALBI: don't like drag} the garment on top of the head. The absence of the hole on the garment leads the dress to generate a force on the head directly dependent on the elasticity of the fabric.  In this way, for each execution we are capable to exploit the different elastic behaviors of fabrics needed to learn the method described in \ref{sec:method}. In particular, the data need to achieve this goal are sequences of meshes with the related force feedback perceived at the end effector of the manipulator. Moreover, we assume that the recording starts while the contact between the body and the garment occours. \\

\subsection{Real-World data collection}
% Real world data collection
To get the real-world training data required, we replicated the dressing scenario with a plastic head and two Franka-Emika Panda equipped with wide 3D-printed grippers to keep the surface of the grasped sample flat. We gathered 17 fabric samples unevenly elastic of dimensions 23x17 cm. To obtain the ground truth mesh, we placed 25 blue markers arranged as a 5x5 grid. These markers were subsequently extracted form images recorded with a RGB camera recording the top view of the working space, leading to a 5x5 2D triangular mesh. The ground truth force measurements were instead recorded from F/T sensors integrated on the gripper of both arms. {\red should we go more into the details of the processing of the singals?\\
MISSING the length of the execution: either to max force of the robot or before the slipping phase
}


% Simulation data collection
\subsection{Simulation data collection}
To collect the simulated data, we replicated the same task used in real world in PyBullet. To avoid to account for the influece of a full robot kinematic on the recorded end-effector signals, we simplified the set-up by deploying two floating grippers. The allowed actions for these grippers were:  pull the fabric along the y direction, drag the garment on top of a simulated head moving along the z direvtion. 
%The choice of the floating gripper was due to the challenges involved when gathering force feedback deploying the full robot. 
The elastic samples where generated varying the spring, damping and bending parameters of the model. {\red full description of the parameters used in the simulated dataset. Still in generation the final one.

More easy here to obtain 3D meshes...//
number of samples ...
Number of timesteps ...

}

 }
 
 
\end{comment}
 


==> includes/full_paper.tex <==
{\color{teal} \textbf{Paper summary:} Insights into elastic behaviours of Fabric is important for modeling, learning, and manipulation :
\begin{itemize}
    \item Fabrics behave very different dynamically depending on their elasticity.
    \item Real Fabric exhibits a wide range of elasticities.
    \item Elasticity is not linear (force over distance)
    \item Pybullet does not model cloth elasticity in accordance to the real world
    \item Models including / learning this properties are better than once that don't (connected to context)
    \item Graph neural networks are a good candidate to model
    \item We \textbf{validate} using a GNN for a mummification task.
\end{itemize}
}



\section{Introduction}
{\color{teal}
Motivate why elasticity matters for fabric manipulation etc. (short (half page))
\begin{itemize}
    \item Why is it relevant? \cite{erickson2018deep}
    \item Why hasn't it been done in fabric manipulation so far?
    \item Why is there simulator real world mismatch?
    \item List of contributions of the paper
\end{itemize}

}




\section{Preliminaries}
{\color{teal}
Here we give the reader the needed background knowledge about fabrics, construction techniques, elasticity etc.
\begin{itemize}
    \item General concept of mechanical properties of deformable objects
    \item How this properties are determined in fabric (construction techniques + yarn material)
    \item How elasticity is measured/modeled
    \item Elasticity curve of fabric sample that gets ripped (different phases of elasticity highlight the non-linearity)
\end{itemize}
}

{\bf Definitions.} \textit{Fabrics} (or textiles) are a special kind of deformable objects. Fabrics are usually a highly deformable 2D structure made out of one-dimensional yarn arranged in a specific pattern. {\color{brown} AK: Garments/clothes are deformable objects, and they are 3D. Fabric is a 2D material (of which garments are made of) that gives these objects a deformability property.} The arrangement of individual yarns through, for example, weaving or knitting, is called a \textit{construction technique}. The material of the yarn ({\color{red} EXAMPLE}) as well as the construction technique determines the dynamic behavior of a fabric. A textile taxonomy, introduced in {\color{red} CITE ALBERTA IROS}, highlights the role construction techniques play in the dynamic behavior of fabrics.
{\color{red} Short recap of construction techniques and yarn material effects}

Textile strength as well as its stretching properties are of particular importance for fabric manipulation. Many modern fabrics contain elastomers to make them more elastic/stretchable. An elastomer such as elastane is often mixed with a traditional fiber material such as cotton to achieve the desired elasticity of certain fabric types. {\color{red} Should we open the can of recovery after stretch ?? }
Fig.~{\color{red} REF} illustrates a tensile strength test curve of a fabric made of {\color{red} DETAILS}. The curve consists of $4$ distinct phases that determine the elasticity of the fabric. {\color{red} EXPLAIN FIGURE 1}

For modeling this behavior, either in a physics simulation environment or with predictive models, a number of approaches have been considered.
Pure elastic deformations are described by the Hooke's law. However, due to the complex geometry of construction techniques, clothes often have a complex and non-linear behavior. \cite{wang2011data} proposed a piecewise linear model to approximate non-linear deformations under an assumption of low levels of stretching, which has a limited practical use.
\cite{breen1994predicting} represented the fabric as a set of particles at crossing points of the threads, where the internal dynamics was ruled by bending energy equations. Albeit directly considering a construction technique, the method lacks generality as it is limited to a plain weave technique.  \cite{eberhardt1996fast} extended this approach to cloth-specific properties such as elastic hysteresis and air resistance. Particle models, however, struggle to model net forces due to the lack of links between particles and are resolution dependent. Alternative approaches that overcome these limitations are non-linear continuum models, where textile surface deformations are described through non-linear Green-Lagrange strain tensor derived from elasticity theory \cite{terzopoulos1987elastically}.  Often these methods linearize the elastic model within a short deformation range assuming small strain regimes \cite{etzmuss2003fast, miguel2012data}. However, linear approximations lose accuracy with large deformations and with clothes high strain are important to consider. High strain might happen near garment seams or when parts of the fabric are physically constrained. To face large displacements, more complex constitutive models such as the Neo Hookean or the St. Venant–Kirchhoff ones were used to to derive non linear hyperelastic relations \cite{boonvisut2012estimation,clyde2017modeling, miguel2016modeling}. 
%Another example is  model, that adopts a cubic tensile force-deformation relationship to better represent non linear tensile force-deformation behavior \cite}.

The flip site do trying to acuratly model this behavoir is to measure it in real world applications, often done for quality control or to gain a better understanding into the proerties of fabrics employed.
The first objective method to evaluate mechanical properties of fabrics was defined in Tokyo and it is nowadays known as Kawabata Evaluation System (KES) \cite{kawabata1989fabric}. This system is a standard set of fabric measuring equipment that can measure the bending, shearing and tensile properties of cloth by evaluating what force or moment is required to deform a fabric sample. Similar specifications are provided by FAST \cite{minazio1995fast} but with a cheaper set-up than the previous one. However, these instruments are very complex and limited in their evaluations \cite{luible2008simulation}. A more simplified set-up is presented similarly in two works \cite{wang2011data, miguel2012data}, were they draw inspiration form biaxial tensile method in literature that is stretching simultaneously two orthogonal elastic directions. These methods however require complex set ups and constrained environments. Moreover, they focus on measuring the low stress mechanical response of  of fabrics which involve small deformations. 
For robotics application these assumption are often violated. 




\section{Elastic Behaviors of Fabrics - Real and Simulated}
{\color{teal}
Here we highlight the elastic behaviors of real world fabrics vs. behavior in Pybullet. (Force figures next to each other (real/ Sim))
\begin{itemize}
    \item Real world fabrics have a wide range of elastic behaviors
    \item As discussed before the behavior is non-linear
    \item The behavior is different from simulation (last phase explicitly).
\end{itemize}
}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{images/profiles_rw_and_sim.png}
    \caption{{\color{violet}Different force profiles extracted from different samples, both for simulation and real world. We can see variation both in magnitude and in shape of the curve, a complex model is required.}{\color{red} change unit measures, put downsampling size. Pybullet with FEM}}
    \label{fig:force_profiles}
    \vspace{-0.2cm}
\end{figure*}

In robotics, many of the aforementioned aspects that make elastic properties of clothes complex and diversified are often overlooked. One reason is the fact that elasticity is a property unobservable from static feedback (single image, single pointcloud), that requires non-trivial manipulation strategies to be retrieved by the robot's sensors {\color{red}(Regrasping problem)}. In this sense, the lack of dexterity of current robots slows the process of understanding how this property becomes relevant in certain applications in textile industries and assistive dressing. Our aim is to contribute in filling this gap by informing the robotics community on how these behaviours appears and influence certain robotic manipulation tasks involving clothes, as well as suggesting how current simulators for deformable objects lack in considering and modelling these properties. {\red{(maybe this sentence should be moved at the end of previous section, or end of introduction.)}}

% Motivation and contribution
The stress-strain curves of fabrics could be divided in three regions: region of initial resistance to deformation, a region of low deformation, and a region of high deformation \cite{breen1994predicting}.  In the low deformation region the assumption of linear elasticity yield reasonable cloth-like behaviors. The same does not hold for the initial-resistance and high deformation regions and usually require to be approximated with non-linear energy functions. The mechanical behavior of the cloth throughout its range of deformation is therefore non-linear, especially during the initial/high deformation regions.
{\red MW: The motivation figure we discussed would fit well to this discussion imo.}

% The interaction strategy that we implement to retrieve elastic information is by using a pulling action, which we define as .... {\color{red} (definition of our pulling action, force feedback perceived on the end effectors of the robots.)}. 
% {\red MW: The bandage wraping and hat examples could be invocet to say that there are task that operate specificly with the elastic behavior (also the bag wrapping example form teh airport - say about )}

Analyzing the real world force data collected by pulling different garments with the robotic setup visible in Figure \ref{fig:streching_explanation}, we can see how different textile samples show complex and diversified stress-strain trends {\red{(Figure \ref{fig:force_profiles} - left)}}. This variant behaviour is more marked for highly elastic materials, suggesting that a more complete taxonomy than the "rigid-elastic" binomial is needed for clothes manipulation. {\color{red} Add a bit more explanation about complex elastic behaviours in textiles, cite some references}.

 \begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{images/stretching_direction2.png}
  \caption{(Top) Flat 3D-printed grippers holding wool sample. The yarn direction coincides with the pulling direction. FT sensors are mounted on the wrist of the manipulators. (Bottom) Schematic example of \textit{pull} and \textit{twist}.}
   \label{fig:streching_explanation}
\end{figure}

On the other hand, commonly used models in simulators of clothes do not implement these types of behaviour. {\color{red} (One sentence about the models used) Most of the analytical methods used to model deformable objects in robotics simulators are based on mass spring models, while others are based on PBD/FEM {\red{(CITE)}}}. We performed the same pulling experiment on {\color{red} Pybullet/alex simulator} retrieving the stress-strain profiles. In {\red{Figure \ref{fig:force_profiles} - center and right}} we can see how the force profiles collected for different samples show different trends than the ones from the real data, mostly in the modelling of the final region of the stress-strain curve {\color{red} (redo these plots with settings as similar as possible to real)}. 

We argue that embedding these elastic behaviours in currently used robotics simulators can be useful to improve control tasks or dynamics prediction ...............



\section{Learning elastic behaviors}
{\color{teal}
Here we show that models modeling elastic properties specificly are stronger than ones that don't. And that graphs are a promising model to do that.
\begin{itemize}
    \item Motivation of why models more real are better (with citations)
    \item Motivate why GNN's are a natural choice with many advantages as a first step towards this
    \item Introduce the model details / Context motivation and definition
\end{itemize}
}

{\red{Missing point 1 and 2: Our models are based on graphs because of by the extensive use in simulators. We also open to the possibility of using these models in real to sim settings, learning a graph representation informed by these properties that can be used in simulation and so on (reprise in Future work).}}



We formulate the problem as a graph dynamics prediction task and we exploit the force feedback sensed at the grasping points of the cloth to account for the different elastic properties of the textiles that the robot manipulates. 
% Modelling the cloth using a graph is a natural choice, given the extensive use of these models in computer graphics and simulators {\red{(CITE)}}. These models allow to encode peculiar properties of the represented object in nodes and edge features, and account for them  the behaviour of the object

Let $G^{t}=(V,E)$ be a static undirected graph composed by a single connected component representing a textile sample at a certain instant in time, where $V$ is the set of nodes and $E$ the set of edges, where its nodes features $x^{t}_{v \in V} \in \mathbb{R}^3$ represent the geometric displacement of the graph in the Euclidean space. Let $F^{t}$ be the force perceived at the two end-effectors of the robot and $a^{t}_{v} = \Delta x_{v} \in \mathbb{R}$ the action applied at the nodes grasped by the robot, causing the change $x^{t}_{v}= x^{t-1}_{v} + a^{t}_{v}$ to their features. The action $a^{t}_{v}$ is propagated through the edges of the graph via a recursive message-passing {\color{red} [reference]} obtaining the actions $a^t_i$ for the remaining nodes: 

\begin{equation}\label{dyna}
 a^t_i = g\left( \sum_{s\in N(i)} f_{ \{ i, s\}}(a^{t-1}_i, a^{t-1}_s)   \right)
\end{equation}
Here, $N(i) = \{s \in V \ | \ \{i,s\}\in E \}$ denotes the neighbours of $i$ in $G$. 

Given a dataset $\mathcal{D}$ where each datapoint $p \in \mathcal{D} = (G^t, G^{t+1}, F^{t}, F^{t+1}, a^t)$, we train a \textit{Dynamics prediction model} $\lambda$ that learns to approximate the dynamics of the next state by minimizing the error between the predicted and the ground truth tuple $(G^{t+1}, F^{t+1})$. The prediction consists in both the graph at the next state and the force, adding the possibility for the model to be used in applications requiring a constraint over the forces exerted on the deformable objects (e.g. assistive dressing). We can write the loss of the system as:
\begin{equation}
\mathcal{L}(\theta) =  \mathbb{E}_{p \in \mathcal{D}}\left[ \  d(\lambda(G^t, F^t, a^t), \  (G^{t+1}, F^{t+1}) \ \right].
\end{equation}

where $d$ is the MSE loss between the predicted and ground-truth graphs and forces and $\lambda$ is a message-passing graph neural network which implements the propagation dynamics in Equation \ref{dyna} {\red weird reference} as
\begin{equation}\label{gnn}
 h^T_i = \phi\left( \sum_{s\in N} W_{i,s} \odot f\left( h^{T-1}_i, h^{T-1}_s \right)   \right) \forall i\ \in V
\end{equation}
for $T$ propagation steps, where $W_{i,s}$ is the adjacency matrix of the graph and $\phi$ is a multi-layer perceptron.

% The prediction of the next state is then:
% \begin{equation}\label{lin}
%  \lambda(G^{t+1}, F^{t+1}) = lin\_proj(h^T)
% \end{equation}


\begin{figure}[h!]
  \centering
  \includegraphics[width=.8\linewidth]{images/GNN_condition_on_force.png}
  \caption{\color{red} Image of the full model with propagation steps etc.
  {\red In this fig it predict delta F not F_p? }
  }
  \label{fig:system}
\end{figure}

We use three different approaches to condition the dynamics prediction task to the force feedback. The conditioning is implemented by appending the force information to each node of the graph.
% We divide the approaches in two main classes: a) we condition the prediction of the next step to the force perceived at the previous step. b) we condition the prediction steps to the force profile of a full interaction collected before the dynamics prediction task. 
% For a) we assess the following types of conditioning:
\begin{itemize}
    \item \textit{$\Delta F$ conditioning:} where $F^{t}$ in Equation \ref{gnn} is $ \Delta F^t = F^{t-1} - F^{t-2} $.
    \item \textit{$\Delta F_{profile}$ conditioning:} where $F^{t}$ in Equation \ref{gnn} is a vector containing the downsampled force profile between $F^{t-1}$ and $F^{t-2} $.
    \item \textit{Context conditioning}: where $F^{t}$ in Equation \ref{gnn} is a vector containing a downsampling of the whole force profile of a previous interaction with the cloth, in the form of a pulling action. In the \textit{context} we also include the displacement information by appending also the action $a^{t}_{v}$.                                                                                                                                 .
\end{itemize}


\subsection{Baselines}

{\color{red}We implement N baselines for comparison. GNN baseline force \& no force - MLP baseline for forces}

\begin{figure}[h!]
  \centering
  \includegraphics[width=.8\linewidth]{images/GNN_baseline}
  \caption{\color{red} This image should have all the images of the different baselines together (or we just remove it)}
  \label{fig:system}
\end{figure}



\section{Related work}

{\color{teal}
The main classes of related works that we present are:
\begin{itemize}
    \item Learning elastic properties
    \item Learning dynamics with graph neural networks
\end{itemize}
}

Learning elastic models using real world data is still under explored. The interest comes from the chance to face the challenge of partial observability. Some interesting results were obtained from  \cite{li2019propagation}, where they propose Propagation Networks (PropNet) to learn dynamics with only sensor measurements. However these networks were entirely trained in simulation. Recently, \cite{valencia2020combining} combined IN and PropNet to learn dynamics of deformable object entirely from pointclouds.

Graph neural networks have shown to be a particularly powerful framework in the context of learning mesh-based dynamics, being employed in a variety of complex domains \cite{georgousis2021graph, chang2016compositional}. \cite{battaglia2016interaction} proposed Interaction Networks (INs) to learn a physical engine to capture the underlying physical interactions by modeling them as a complete graph over the particles. This model can then be used to predict future states of the object. However, INs cannot handle propagation of forces as they consider just local information. To overcome this problem \cite{li2019propagation} proposed propagation networks (PNs) which enables instantaneous propagation of forces by multiple message passing. 
In a previous work, \cite{li2018learning} used GNNs to learn particle-based  dynamics by using a graph that dynamically changes through time instead of being static, that allows the model to approximate more complex dynamics and interactions involving discontinuous functions (e.g. contact). Moreover, they introduce hierarchy to deal with long-range dependencies. \cite{pfaff2020learning} learned a mesh-based simulator with GNNs, where they adopt an adaptive remeshing algorithm to increase the scale of the representation when needed. This method, differently from the ones previously mentioned, considered textiles as deformable objects and showed good results in modeling clothes behaviors. However, the focus of these models is on node features or mesh structure rather then the relevance of edges features.


\section{Evaluation}
{\color{teal}
Here we show that the claims/motivations hold by doing experiments.
We highlight the model that models elasticity is stronger on a dynamic prediction task (comparison in simulation only). We validate that the model is usable an a robotic mummification task (no comparison)
\begin{itemize}
    \item We show that a model that learns either the mean or a single "elasticity" profile is worse than a model that uses the "context" (basically adopts to the different profiles before predicting A non graph example would be adopting the k of a linear model by first calculating it using the "context")
    \item Validate GNN on mummification task by doing it.
\end{itemize}
}

==> includes/old_files/00_introduction_old.tex <==


\section{Introduction}
\begin{comment}

{\red Introduction of the problem and the contributions of the paper.}
{\color{teal} 
\begin{itemize}
    \item Relevance of fabric properties in robotic manipulation: assistive dressing (elasticity), keep the grasp (friction).
    \item Complexity of taking into account all these properties and the variety of mechanical behaviors they generate. Introduction to material and construction techniques.
    \item Very good analytical models are available, from the yarn level discription up to the visual effect like wrinkles. However these models require fabrics parameters to be known a priori and identification techniques might be expensive or unfeasible in robotics environments.
    \item Humans don't need all these information but they are still succesful, the same could be achieved via neural networks.
    \item Elasticity for this initial project, but it's an unobservable property in static scenarios. Force response are used in general identify it
    \item GNN are are good models with the right inductive bias to model mesh particles and force dynamics.
    \item We define an elastic context inspired by previous approaches to condition the model and make it robust to changes in elastic properties.
    \item We evaluate this approach both in simulate and real scenarios, leveraging the knowledge from other communities.
\end{itemize}
Therefore the contributions are:
\begin{itemize}
    \item (Inform the community about the complexity of the problem and it shouldnt be overlooked. Not mentioned explicitly though.)
    \item We define an elastic context for fabrics and show how it can be used to performe force predictions
    \item We highlight the mismatches between real-world cloth behaviors and simulated ones.
\end{itemize}
}

Motivated by recent developments in artificial perception, cognition and control, robotic systems have found widespread use in multiple scenarios such as in medical~\cite{peters2018review}, educative~\cite{belpaeme2018social} and industrial settings~\cite{ji2019industrial}. In particular, these developments have allowed the use of robots as suitable tools for assisting humans in complex tasks such as industrial collaboration~\cite{vysocky2016human} and assistive dressing~\cite{klee2015personalized,kapusta2019personalized}. In order to be effective in such tasks, robots require complex controllers that allow the precise manipulation of highly-deformable objects, such as clothes and textiles, whose dynamics can be shaped by the material of the yarns and the way they are arranged to construct fabrics~\cite{longhini2021textile}. 


{\al 
Intro\\
.....\\
In robotics, many of the aforementioned aspects that make elastic properties of clothes complex and diversified are often overlooked. One reason is the fact that elasticity is a property unobservable from static feedback (single image, single pointcloud), that requires non-trivial manipulation strategies to be retrieved by the robot's sensors {\color{red}(Regrasping problem)}. In this sense, the lack of dexterity of current robots slows the process of understanding how this property becomes relevant in certain applications in textile industries and assistive dressing. Our aim is to contribute in filling this gap by informing the robotics community on how these behaviours appears and influence certain robotic manipulation tasks involving clothes, as well as suggesting how current simulators for deformable objects lack in considering and modelling these properties.\\
...

}


% Description of modeling deformable objects dynamics
A tough challenge in deformable object manipulation is represented by the definition of the underlying dynamics of the object. While for rigid objects knowing its shape, friction and mass) might be sufficient to describe its dynamics {\color{red}(backup  this  sentence)}, for deformable objects the definition of a fixed set of parameters is often challenging 
When dealing with fabrics, the complex dynamics of deformable objects are enhanced by the material of the yarns and the way they are arranged to construct fabrics \cite{longhini2021textile}. This information is relevant for many robotics tasks where active interaction with the cloth is involved and could play a fundamental role in improving dynamics models used for model-based controllers in important robotics tasks like assisted dressing \cite{kapusta2019personalized} {\red cite Zackory maybe}. Elasticity, however, is an unobservable property in static states and require specific interactions to be identified.
Industrial approaches adopt highly sophisticated set-ups to define fabrics parameters such bending, shearing, damping \cite{kawabata1989fabric, minazio1995fast}. These solutions use constrained environments that are not well suited for robots. A promising direction to overcome this limitation is proposed in a recent work \cite{longhini2021textile}, where it was shown that force feedbacks could be valuable measurements to extract elastic-related information.
%In \cite{longhini2021textile} it was shown that force feedbacks could be a valuable measurements to extract relevant infomation, since it helps in the classification of materials and construction techniques.
Current robotics applications, however, overlook the challenges of modeling elastic behavior of fabrics. In some cases, they even avoid it losing generalization of their approaches {\red write it better}.

% There are different ways to model textiles
% Analitical
% Textile engineering perspective
% Computer graphic perspective
% Data driven
% Limitations here are the computational complexity or realism
Modeling elastic objects dynamics can be approached from different point of views. Analytical methods can be very accurate in describing non-linear cloth behaviors, but they have the disadvantage to be complex and expensive to compute.  Moreover, they are limited by the requirement of knowing all the properties of the object a priori in order to predict its dynamics. In many real world applications the unknown attributes of deformable objects pose an overwhelming challenge for these off-the-shelf approaches. Humans, however, do not have a detailed physics knowledge of the objects they manipulate. Similarly, black-box model like neural networks are a viable way to model deformable objects dynamics without predefined parameters.
Learned models have shown to be able to quickly adapt and better generalize in new scenarios when object parameters are unknown, leading to an increase of interest in these data-driven approaches to learn dynamics for robotics applications. Learning-based models that are commonly used do describe particle systems are Graph Neural Networks (GNNs) \cite{battaglia2016interaction, li2019propagation}. The inductive bias of propagation of dynamics information through the graph structure allows to represent rich physical states with interaction particles and to approximate complex dynamics by learned message passing among nodes \cite{sanchez2020learning}. 
.....

In this work we focus on a strategy to encode elastic-related infromation in representation of textiles useful for robotic manipulation




% Comparison between computer graphic and textile engineering communities

Computer graphics is not interested on the precision of the dynamics model, but on the macroscopic properties of the cloth surfaces. Realism overcome physical accuracy. 

Fast simulation is required. Textile engineering instead aims for precise modeling of microscopic behavior. They want to unerstand non-linear behaviors for accurate modeling of clothes. However, bringing together the expertise of the two communities brought to the development of valuable solutions for both.
In robotics community...

Our initial study focus on  learning and modeling small scale interactions of real-world fabric samples. 


\end{comment}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{images/different_elastic_meshes2}
  \caption{Visualization of  two different elastic samples that reach the same force response at different stages of the manipulation. {\red still not the final image.}}
  \label{fig:different_meshes}
\end{figure}

==> includes/old_files/01_introduction_oldtex <==
\section{Introduction}


% Introduction 
{\al 
% Introduce the problem of modeling deformable objects

A tough challenge in deformable object manipulation is represented by the definition of the state of the object. While for rigid shapes knowing the pose of the center of mass is sufficient to describe their position and orientation in space, for deformable objects the definition of a fixed configuration of points is not enough. Therefore, understanding how to model them is an important preliminary step to perform autonomous robotic manipulation tasks with more dexterity. 
{\color{red} MW: We will fix the intro when we have decided on where the contribution lies}

% go into the details of the anisotropies from IROS
\subsection{Textile's unobservable properties}
When dealing with fabrics, the complex dynamics of deformable objects are enhanced by the joint effect that treads materials and construction techniques have on textile characteristics \cite{longhini2021textile}.
{\color{red} MW: Should first introduce the conzept of threads or construction techniques before using it.}
Construction technique especially, influence both structural and mechanical properties and is the what dictates the fabrics mechanical behavior rather than the material of the yarn \cite{poincloux2018geometry}.
{\color{red}MW: Is this true? the material still plays a big role right (elastan for example) (We should hedge this claim imo}
Knitted fabrics are usually very elastic, while woven fabrics do not stretch equally in all directions
{\color{red}MW: I would not invoce the anisotropy, can we just say woven steches less or something like that?}
. This information is relevant for many robotics tasks where active interaction with the cloth is involved and could play a fundamental role in improving dynamics models used for model-based controllers in important robotics tasks like assisted dressing \cite{kapusta2019personalized}. 
However, current robotics applications assume the fabric to be homogeneously elastic {\color{red}(in this work we do it as well)}. 
{\color{red}MW: I think current techniques do not consider elastisity at all? and if they have it set to one elastsity no matter the fabric/garment}
In fact, elasticity is an unobservable property {\color{red}MW: mmm it's unobservable in a static state, we should be more specific as later you cite papers triyng to estimate it from video.} that is inferable only by interaction with the deformable object (and graphs?). 
In \cite{longhini2021textile} it was shown that force feedbacks could be a valuable measurements to extract relevant infomation, since it helps in the classification of materials and construction techniques {\color{red}(this is important to motivate the use of force conditioning for the whole method section). 
\begin{itemize}
    \item Extend reasoning about textile properties (ICRA ws) and especially elasticity. 
    \item another thing to keep in mind is that 
    \item Global VS local properties, where elasticity is global but there could be a connection to local properties (like the anisotropy but we're not going to mention it) MW: I don't thenik we need to invoe that for this work
\end{itemize}
}.

% Here, always from IROS, explain that forces are relevant to identify these characteristics


% From here dig a bit more into the representation, from physics based models to learned ones GNN
\subsection{Textile representation - discussion on modeling}
To reduce the complexity, geometric representations such as particles or meshes are often used as a discretization of a deformable object \cite{yin2021modeling}.  
Various methods to model deformable objects dynamics are grounded on physics-based modelling.
%, such as Mass-Spring Models and Finite Element Method (FEM). 
A common example is Mass-Spring Models, which consider deformable objects as a mesh where in the edges is encoded the spring information. Position-based Dynamics instead is a mesh-free method describing objects as a discrete system of particles, but it struggles in modeling force effects due to the lack of links between particles. A third modelling approach is Finite Element Method (FEM), a standard computational method for continuous mechanic problems that discretizes the object as a mesh that is suitable to define a constitutive model which relates stress and deformation of a specific material. 
These simulation approaches, however, are limited by the requirement of knowing all the properties of the object a priori in order to predict its dynamics. 
{\color{red}MW: FEM is also slow as fuck}
In many real world applications the unknown attributes of deformable objects pose an overwhelming challenge for these off-the-shelf approaches.
Learned simulator instead are able to quickly adapt and better generalize in new scenarios when object parameters are unknown, leading to an increase of interest in these data-driven approaches to learn dynamics for robotics applications. Learning-based models that are commonly used are Graph Neural Networks (GNNs), which have emerged as a particularly useful framework able to represent a variety of irregular domains \cite{battaglia2016interaction, li2019propagation}. {\color{red} MW: this makes it sound as 5 and 6 are simulators that are bsed on learning? Is this the case???}
The inductive bias of propagation of dynamics information through the graph structure allows to represent rich physical states with interaction particles and to approximate complex dynamics by learned message passing among nodes \cite{sanchez2020learning}. 
{\red What we are doing differently form these approaches is that we're learning the models from Real World data in order to better replicate the textile dynamics. WHY IS THIS AN ADVANTAGE? For robotics tasks, because it's a textile model that can be obtained from the robot through perception. However, we assume the vision part resolved (that is obtaining the mesh from vision. It can be extended in the future with Zehang work from pointclouds.)}

{\red
DANI:
\begin{itemize}
    \item Discussion on how these models can be used for robotic applications rather than the one used usually for deformable objects - WE USE IN SIMULATION MASS-SPRING MODEL AND WE SHOW WITH REAL DATA THAT ITS NOT EXACTLY THE SAME
\end{itemize}
}
{\red Should we make a clear distingion betwenn "normal def objects and clothing (highly deformable?}

\subsection{Robotics}
{\red Explain better this concept...}
Computer graphics is not interested on the precision of the dynamics model, but on the macroscopic properties of the cloth surfaces. Realism overcome physical accuracy. 
{\red How is Realism diffrent from physical accuracy? the animators are concenred that it LOOKS realistic and take many shortcuts to achive this wich makes the handcrafted animation stuff not suitible for a simulation context (rendering takes foever and it's a predetermind scene.}
Fast simulation is required. Textile engineering instead aims for precise modeling of microscopic behavior. They want to unerstand non-linear behaviors for accurate modeling of clothes. However, bringing together the expertise of the two communities brought to the development of valuable solutions for both. We should do the same in robotics in order to learn deformable object representations that can be adopted to control real robots.
Our initial approach starts form learning and modeling small scale interactions of fabric sample, that in the future can be aggregated to generate macroscopic behaviors.
{\red MW: I like the invocation of this diffretn communitys and we should introduce them and say where robotic fits and that it needs to combine the two blabla.}

\subsection{Goal/ contributions}

% Therefore the goal is ....
The goal of this paper is to learn how to improve robots' perception skills by learning textile models by observing and interacting with them.
{\red MW: didn't we want to imporve the modeling? not the perception?}
In addiction, we want to show the gap between real world and simulated textile models such as the mass-spring model and the one used by pybullet. {\red MW: The models need to be more prevalient as they are now a core contribution.} {\red}

% And to achieve this we ....
To do so we collected simulated and real data of various elastic textile samples. Both datasets are composed by sequences of meshes and force feedbacks collected while pulling the samples. These data were then used to compare the performances of X dynamics predictors to evaluate the relevance of the elastic information.

% Our final contributions are ...

{\color{red} Change:
We summarize the contributions as follow:
\begin{itemize}
    \item We investigate how elastic properties influence the dynamic behaviour of textiles and showcase on simulated data how these behaviours influence dynamics prediction tasks. 
    \item We collect a dataset of real textile samples using a bi-manual robotic manipulation setting.
    \item We show the differences between  real world textile dynamics and simulated ones.
    
\end{itemize}}

}

{\color{red}
%A tough challenge in deformable object manipulation is represented by the definition of the state of the object. While for rigid shapes knowing the pose of the center of mass is sufficient to describe their position and orientation in space, the definition of a fixed configuration of points is difficult to specify for deformable objects such as fabrics. Therefore, understanding how to model them is an important preliminary step to perform autonomous robotic manipulation tasks with more dexterity. To reduce the complexity, geometric representations such as particles or meshes are often used as a discretization of a deformable object \cite{yin2021modeling}.  However, even if a good representation is given, modelling dynamics of fabrics remains a complex task due to their infinite degrees of freedom.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=.8\linewidth]{images/system_setup.png}
%   \caption{{\color{orange}System setup: Two 7 DoF Franka Emika Panda arms with force-toque sensors on the wrists, pulling a textile sample. }}
%   \label{fig:system}
% \end{figure}

%Various methods to model deformable objects dynamics are grounded on physics-based modelling. A common example is Mass-Spring Models, which consider deformable objects as a mesh where in the edges is encoded the spring information. Position-based Dynamics instead is a mesh-free method describing objects as a discrete system of particles, but it struggles in modeling force effects due to the lack of links between particles. A third modelling approach is Finite Element Method (FEM), a standard computational method for continuous mechanic problems that discretizes the object as a mesh that is suitable to define a constitutive model which relates stress and deformation of a specific material. 
%These simulation approaches, however, are limited by the requirement of knowing all the properties of the object a priori in order to predict its dynamics. In many real world applications the unknown attributes of deformable objects pose an overwhelming challenge for these off-the-shelf approaches. Learned simulator instead are able to quickly adapt and better generalize in new scenarios when object parameters are unknown, leading to an increase of interest in these data-driven approaches to learn dynamics for robotics applications. Learning-based models that are commonly used are Graph Neural Networks (GNNs), which have emerged as a particularly useful framework able to represent a variety of irregular domains \cite{battaglia2016interaction, li2019propagation}. The inductive bias of propagation of dynamics information through the graph structure allows to represent rich physical states with interaction particles and to approximate complex dynamics by learned message passing among nodes \cite{sanchez2020learning}. 
}

%When dealing with fabrics, the complex dynamics of deformable objects are enhanced by the joint effect that treads materials and construction techniques have on textile elastic properties \cite{longhini2021textile}. Different combinations of these two characteristics can lead to highly diverse dynamics and anisotropic properties. Therefore, the information relative to stretching attributes could play a fundamental role in improving dynamics models used for model-based controllers in important robotics tasks like assisted dressing \cite{kapusta2019personalized}. However, current representations of fabrics do not take in consideration different anisotropic elastic properties of the cloth. {\color{orange}(put more emphasis on this paragraph and continue discussion)}




==> includes/old_files/02_related_work_old.tex <==
%\section{Preliminaries and Related Work}
\section{Background and Related Work}
\label{sec:preliminaries}

% {\red Provide most relevant information about fabrics properties, analytical models, identification techniques and robotic perspective}

% {\color{teal} 
% \begin{itemize}
%     \item Fabric mechanical properties (like elasticity, surface friction, plasticity) are complex. The main influencing factors are materials and construction techniques.
%     \item These behaviors can be modeled trough analytical models thanks to two pioneer communities: computer graphics and textile engineering. 
%     \item these communities had different goals in mind. Fast Computation / Accuracy trade off.
%     \item These models require specific parameters for each samples. These parameters can be obtained with old school techniques. Some more advanced techniques are less expensive but still require constrained environments. 
% \end{itemize}
%}

We structure the related work along elastic properties of textiles, analytic and data-driven approaches towards encoding these, and work in robotics regarding manipulation of deformable objects. Recent reviews provides an overview of flexible deformable objects and their use in dexterous robotic manipulation \cite{hou2019review, yin2021modeling}.


\subsection{Elastic Properties of Textiles}
{\note this can be summarized and most of these things can be pointed to the textile paper, and this section could be blended with the next one}
Properties such as elasticity, surface friction, flexibility of textile items are mostly determined by the yarn material the textile is made of and its construction or production technique. The construction technique is usually woven or knitted. Thus, the elastic behavior of the textile stems from both the construction technique and elastic property of the yarn material and their effect may be impossible to identify solely using robot's force-torque sensor {\note this has to be removed}. In modern textiles, the raw material such as cotton or wool is blended with elastometers such as elastane making the yarn intrinsically more flexible and affecting its elasticity~\cite{uyanik2019strength}.  
 
The construction technique determines how the yarn threads are interlaced or interloped - woven textile such as jeans is hard, has high friction and it is almost not elastic in comparison to very elastic knitted textiles.
Thus, woven textiles are produced with two sets of tightly interlaced yarns that make the textile rather rigid. Knitted textiles, instead, are made with one interloped thread. The loops in the knitted textile generate open spaces between the threads running in parallel, making it more stretchable than woven textiles. A textile taxonomy introduced in \cite{longhini2021textile} describes in more detail these construction techniques.

\subsection{Analytical Elastic Models}
Analytical models of textiles are usually based on physics-based modeling and geometric representations such as particles or meshes \cite{yin2021modeling}. {\note Here better description and introdution to PBD} Models commonly rely on Position-based Dynamics (PBD) using a discrete system of particles and modelling their displacement. Particle based approaches, however, struggle to model net forces and are resolution dependent \cite{breen1994predicting,eberhardt1996fast}. Mesh models overcome these problems by encoding the interaction between the particles in the edges of the mesh. In mass-spring models, the edges represent springs following the Hooke's law to encode pure elastic relationship \cite{wang2011data}. Damping, bending and shearing factors are also modelled to reproduce more complex behaviors.  Linear approximations however, lose their accuracy with large deformations. When modeling textiles, high strains cannot be ignored as they may occur  near garment seams or when parts of the textile are physically constrained. To deal with large displacements, more complex constitutive approaches such as the Neo Hookean or the St. Venant–Kirchhoff models are use to encode non linear hyperelastic relations \cite{boonvisut2012estimation,clyde2017modeling, miguel2016modeling}.  These models have the advantage of being more realistic than the mass-spring models, but their computational complexity is not suitable for fast simulations. In robotic manipulation tasks, task-specific and reliable textile representations are often favoured over a precise description of all possible mechanical behaviors of the textiles \cite{mcconachie2020interleaving}. Finding a suitable trade-off between the model accuracy and numerical efficiency is therefore of fundamental importance \cite{marinkovic2019survey}.


\subsection{Learning Textile Representations}
Analytical models require knowledge of textile parameters to model the  textile dynamics. This may be difficult in robotic applications when a robot encounters a textile item for the first time.  Despite the effort to simplify the complex measurement tools used in textile engineering, the estimation of textile parameters remains highly engineered \cite{wang2011data, miguel2012data}. Black-box models like neural networks provide a viable solution to model dynamic behavior without the exact knowledge of all the parameters. Graph neural networks have shown to be a particularly powerful framework in the context of learning mesh-based dynamics, being employed in a variety of complex domains, including deformable objects \cite{georgousis2021graph, chang2016compositional, lin2022learning}. 
Battaglia,~\etal~\cite{battaglia2016interaction} proposed Interaction Networks (INs) to learn a physical engine to capture the underlying physical interactions by modeling them as a complete graph over the particles. However, INs cannot handle propagation of forces as they consider just local information. To overcome this problem, Li ~\etal~\cite{li2019propagation} proposed Propagation Networks (PNs) which enable instantaneous propagation of forces by multi-step message passing. These approaches have shown excellent results in modeling deformable objects, but they assume the mechanical parameters known. {\note our contribution has to be highlighted} We relax this assumption by proposing the EC. In contrast to prior works, we focus our analysis on the evaluation of the capabilities of a GNN to model force dynamics rather than the spatial position of the nodes in the graph.







% {\al
% % Introduction about fabrics
% Garments/clothes are flexible deformable objects considered as a two-dimensional surface \cite{hou2019review}. Due to their deformable nature, their mechanical properties such as elasticity, surface friction or flexibility are highly complex and vary for every sample. The factors that influence them the most are the yarn material and the arrangement of the yarn fibers over the textile, also called construction technique. The material of the yarn defines how rough the surface of the fabric will be. Moreover, the possible addition of elastometers (such as elastam {\color{red}(CITE)}) can induce a more elastic responses. Elasticity, however, is also influenced by the underlying construction technique, i.e. woven and knitted.  Woven fabrics are produced with two sets of tightly interlaces yarns that make the fabric rigid. Knitted textiles, instead, are made with one interloped thread. The loops in the knitted fabric generate open spaces between parallel lines of the object, making it usually more stretchable than woven fabrics. A textile taxonomy introduced in \cite{longhini2021textile} describes in  more detail the role that construction techniques play on defining fabric behaviors. \\
% % Modeling of these
% %For modeling this behavior, either in a physics simulation environment or with predictive models, a number of approaches have been considered.
% }





% {\al
% How to model fabrics behavior has been an important research question over the past two decades, and the major contribution came from two main pioneers communities: textile engineering and computer graphics. The goal of the former is to seek for a precise analytical model of fabrics capable of describing its complex mechanical behaviors. These analytical methods are usually grounded on physics based modeling, where geometric representations such as particles or meshes are often used as a discretization of the object to reduce the problem complexity \cite{yin2021modeling}. Pure elastic deformations are described by the Hooke's law, which was extended by \cite{wang2011data} to a piece-wise linear model to approximate non-linear deformations under an assumption of low levels of stretching. 
% % Describe non linear
% For what concerns non-linear surface deformations instead, there are mainly two viable solutions. The first one is to use Green-Lagrange strain tensor  derived from elasticity theory \cite{terzopoulos1987elastically}, while the second one is to use complex constitutive models such as the Neo Hookean or the St. Venant–Kirchhoff ones to derive non linear hyperelastic relations  \cite{boonvisut2012estimation,clyde2017modeling, miguel2016modeling}. 

% % Describe peaople going into yarn level


% % Describe computer graphics
% In constrast, the computer graphics community pursues realism and fast computations. Therefore they often preferred simpler models or linear approximation of the non-linear ones mentioned before \cite{etzmuss2003fast, miguel2012data}. For further details about modeling, we refer the reader to the following reviews \cite{jevvsnik2014review, yin2021modeling}
% {\red missing comment about how relevant was for them to join their perspective to reach amazing results.}

% %However, due to the complex geometry of construction techniques, clothes often have a complex and non-linear behavior.  proposed a piecewise linear model to approximate non-linear deformations under an assumption of low levels of stretching, which has a limited practical use.
% %\cite{breen1994predicting} represented the fabric as a set of particles at crossing points of the threads, where the internal dynamics was ruled by bending energy equations. Albeit directly considering a construction technique, the method lacks generality as it is limited to a plain weave technique.  \cite{eberhardt1996fast} extended this approach to cloth-specific properties such as elastic hysteresis and air resistance. Particle models, however, struggle to model net forces due to the lack of links between particles and are resolution dependent. Alternative approaches that overcome these limitations are non-linear continuum models, where textile surface deformations are described through non-linear Green-Lagrange strain tensor derived from elasticity theory \cite{terzopoulos1987elastically}.  Often these methods linearize the elastic model within a short deformation range assuming small strain regimes \cite{etzmuss2003fast, miguel2012data}. However, linear approximations lose accuracy with large deformations and with clothes high strain are important to consider. High strain might happen near garment seams or when parts of the fabric are physically constrained. To face large displacements, more complex constitutive models such as the Neo Hookean or the St. Venant–Kirchhoff ones were used to to derive non linear hyperelastic relations \cite{boonvisut2012estimation,clyde2017modeling, miguel2016modeling}.  
% % Parameter Estimation
% %The flip side of trying to accurately model this behavior is to measure it in real world applications, often done for quality control or to gain a better understanding into the properties of fabrics employed.
% The downside of trying to accurately describe these behaviors, is the need to tune the model's parameters according to the real world fabric responses.
% The first objective method to evaluate mechanical properties of fabrics was defined in Tokyo and it is nowadays known as Kawabata Evaluation System (KES) \cite{kawabata1989fabric}. This system is a standard set of fabric measuring equipment that can measure the bending, shearing and tensile properties of cloth by evaluating what force or moment is required to deform a fabric sample. Similar specifications are provided by FAST \cite{minazio1995fast} but with a cheaper set-up than the previous one. These instruments, however,  are very complex and limited in their evaluations \cite{luible2008simulation}. A more simplified set-up is presented similarly in two works \cite{wang2011data, miguel2012data}, were they draw inspiration form biaxial tensile method in literature that is stretching simultaneously two orthogonal elastic directions. These methods however require complex set ups and constrained environments that prevent these strategies to be easily integrated in robotics manipulation pipelines. 
% %Moreover, they focus on measuring the low stress mechanical response of  of fabrics which involve small deformations. 



% % Limitations here are the computational complexity or realism

% %Modeling elastic objects dynamics can be approached from different point of views. Analytical methods are usually grounded on physics-based modelling, where geometric representations such as particles or meshes are often used as a discretization of the object to reduce the problem complexity \cite{yin2021modeling}.
% %, such as Mass-Spring Models and Finite Element Method (FEM).
% %Approximating complex elastic behavior is often used to deal with small loads. A common example is the Mass-Spring model, which consider deformable objects as a mesh where in the edges is encoded the spring information. Higher strains however do occur even in everyday use of garments and are therefore also important to consider for robotic simulations. For this purpose, Position-based Dynamics (PBD) is a valuable  mesh-free method to desctybe behaviors of a system of particles, but it struggles in modeling force effects due to the lack of links between particles. A third modelling approach is Finite Element Method (FEM), a standard computational method for continuous mechanic problems that discretizes the object as a mesh. This method is suitable to define a constitutive model for non-linear stress-strain relations of a specific material. These models can be very accurate in describing non-linear cloth behaviors, but they have the disadvantage to be complex and expensive to compute. Moreover, they are limited by the requirement of knowing all the properties of the object a priori in order to predict its dynamics. In many real world applications the unknown attributes of deformable objects pose an overwhelming challenge for these off-the-shelf approaches.

% }
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/breakpoint.png}
    \caption{Typical stress curve for manipulation of elastic textile. In the free manipulation phase no forces are exerted on the end-effectors. In the stress manipulation phase the properties of the textile determine the behavior and forces sensed. If the force applied is too large the textile breaks.}
    \label{fig:phases}
\end{figure} 

\subsection{Robotic Manipulation of Textiles}
% \begin{itemize}
%     \item In robotics no need to describe every single particle, the cloth can be discretized as a mesh because we need also to model relationships between the particles.
%     \item The more complex the model the more parameters it requires the more sophisticated the sensors the robot needs to have.{\color{red the more complex system identification or waht do you want to say?}} But in robotics is not necessary to know in detail every single parameter.
%     \item Robotics has the chance to focus on specific tasks instead of modeling general solutions. {\color{red} a general solution would include the specific case right? YES, but it's extremely hard to model it (both analytically and leaning wise)}
% \end{itemize}
% }

%In robotics, cloth modeling can be highly task specific and the focus is more on modeling reliable dynamics that do not need to precisely account for all the mechanical behaviors of fabrics. Many approaches opt to represent only task relevant features of the deformable object with simplified models {\color{red} CITE BERENSON ROPE?}, and focus on tasks where modelling elastic aspects are of limited importance such as grasping, folding or flattening {\red cite maybe a review of tasks}. 
{\note this part can be shortened and maybe blended with the introduction. Another way to propose this section is to merging it with the firs one!}

To analyse the elastic behavior of different textiles, the Stress-Strain test is often employed, where a fixed load is applied to a piece of textile and the displacement, also called elongation, is measured~\cite{kawabata1989fabric, eberhardt1996fast}. 
%Different force loads can be employed, for example using robotic end-effects as proposed in ~\cite{longhini2021textile}, resulting in a textile-specific profile which can be decomposed into three-different stages, as shown in Fig.~\ref{fig:phases}. 
Different force loads can be applied to the textile, for example using robotic end-effectors as done in \cite{longhini2021textile}, resulting in a textile-specific profile which can be decomposed into three-different stages as shown in Fig.~\ref{fig:phases}. In a first stage (\textit{free} manipulation), no stress is introduced on the end-effector as the deformable nature of the textile makes it compliant to the robot movement without any resistance. On a second phase (\textit{stress} manipulation), the textile starts to induce forces on the end-effector and its mechanical properties, such as elasticity, become important to consider. Finally, after a certain textile-specific force, in the third-phase the object reaches a breaking point. 
Often in robotic tasks, objects are manipulated under the \textit{free} manipulation phase. 
For tasks such as assistive dressing, precise modelling of the \textit{stress} manipulation phase can be advantageous to predict when too much force is exerted on the person being dressed or to assure that a specific dressing action is performed correctly \cite{erickson2018deep}. These tasks have been addressed so far with the implicit assumption that the elasticity of different manipulated samples do not exhibit large variations in their dynamics, despite the wide diversity of potential textile suitable to be employed in assistive dressing tasks (such as first-aid bandages, t-shirts, jeans). In this work, we consider the learning of models of textile samples with EC, allowing to generalize to different elastic responses of textiles.


%These tasks have been addressed so far with the implicit assumption that the elastic property can be indirectly inferred when using enough training data as the garment type is normally not changing in these scenarios.
%{\red modify this conclusion}
%However, when considering a wider range of fabrics for tasks in assistive dressing or first aid tasks, like bandaging, the elastic diversity need to be considered. One way to condition the models on specific properties is to first perform a system identification step, by using supplementary sensors such as force-torque, or touch sensors {\color{red} GEL?} to enhance the perception capabilities of the robot. Equipping robots with high quality sensors can be however a costly endeavor. {\color{red} Some conclusion sentence here}


% In robotics, a precise and visually realistic representation for clothes is less needed than in computer graphics, and a mesh-discretization of the cloth to be manipulated obtained from pointclouds or through landmarks is often enough for a robot to accomplish different tasks {\color{red} CITE}. For more challenging scenarios though, as in assistive dressing {\color{red}CITE}, modelling elastic properties can be advantageous, for example to predict when clothes are stretched too much or if too much force is exerted on the person dressed. However, many of the aforementioned aspects that make elastic properties of clothes complex and diversified are often overlooked, and this is also caused by the lack of dexterity of current robots. Augmenting the existing cloth models used in robotics applications to represent relevant elastic properties becomes then important, and one approach is to use supplementary sensors like force-torque to enhance the perception capabilities of the robot {\color{red} CITE}. By then using task-specific data collected with these sensors, the robot is allowed to use the information of the different elasticity from the different garments and possibly adapt the manipulation strategy to them.

==> includes/old_files/06_experiments.tex <==
\section{Experiments }
{\color{teal}

... Details of the models and training parameters used for both the scenarios ...
Models used for the evaluation and the comparisons:
\begin{itemize}
    \item 
\end{itemize}

The goals of the experiments are:
\begin{itemize}
    \item (INTERNAL: To show that our method is capable to learn particles and force dynamics. Not necessary in the final paper)
    \item to show that the conditioning is relevant to improve force predictions
    \item evaluate how the size of the context influence the quality of the prediction
    \item highlight discrepancies between real world and simulation in terms of range of elasticity that can be modeled.
\end{itemize}

}

{\al
To evaluate our method we devised a set of experiments to asses how well our conditioned model is capable to account for different responses of fabric samples with different elasticity. The results aim to show:
\begin{itemize}
    \item the quality of the prediction of the models {\red visualisation and comparison with baselines}
    \item the validity of conditioning the model on elastic information {\red training curves}
    \item the necessity of multi-dimensional context to increase performances {\red rollout results}
    %\item {\red discrepancy between real wold and simulation}
\end{itemize}

We use the following baselines to determine the quality of the results:
{\red ALBI: don't like this way of presenting the modeld. I will change it soon}
\begin{itemize}
    \item \textit{GNN baseline}: standard GNN that predicts the next graph state given the action.
    \item \textit{GNN without conditioning}: GNN that predicts simultaneously the next graph state and the predicted force given the action.
    \item \textit{MLP baseline}: standard MLP that predicts the force given the action
    \item \textit{MLP with conditioning}: MLP conditioned on the elastic context that predicts the force give the applied action.
\end{itemize}

All the models shared the same body-architecture composed by 6 linear layers. For what concern the  graph-prediction and the force-prediction heads,  one linear layer and two linear layers were deployed respectively. All the layers had 32 hidden neurons, and in between the ones not involved on the propagation step of the GNN, we used Rectified Linear units (ReLu) as activation function. The models were trained for 500 epochs and mini batch size of 32. We use ad learning rate of $3 \times 10^{-4} $ and a train/test split of 0.2, while the parameters where optimized using Adam {\red cite}. {\red missing different seeds} All the training objectives and test measures for the forces used mean squared error (MSE) between the model's prediction and the ground truth. For what concern the graph, we used the sum of the squared euclidean distances computed at each node between the predicted ones and the ground truth. This choice helped to mask-out the nodes that during the task execution were fixed because blocked by the head, leading to a more informative loss function.



\subsection{Context evaluation}

\begin{figure*}[!t][h]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/force_context_loss.png}
         \caption{Force loss comparison.}
         \label{fig:force_context_loss}
     \end{subfigure}
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/graph_context_loss.png}
         \caption{Graph loss comparison}
         \label{fig:graph_context_loss}
     \end{subfigure}
\label{fig:test_losses}
\end{figure*}

Figure \ref{fig:test_losses} show the test losses of the four models described above trained with the real-world data. {\red FROM THE VISUALIZATION OF THE PREDICTION It can be observed that our models can predict the next step dynamics.} For what concern the force prediction, it can be observed that both the MLP and the GNN trained without the elastic context can learn to predict the mean force of the dataset. The conditioned models, instead, show the capability to leverage the information contained in the context. Another observation is that in both the scenarios where the models are either conditioned or not, the GNN require less time to reach  convergence. As both the graph and the force dynamics depend on the interactions among the fabric nodes, the bias imposed using a propagation network as the GNN helped to learn and exploit these relationships  like suggested \cite{li2019propagation}. The same reasoning hold for the graph loss, where the information about the elasticity lead the conditioned model to learn faster the graph prediction. 

%{\red plot on the figure the error that there if from the mean of the dataset!!!}



}



==> includes/old_files/06_experiments_old.tex <==
\section{Evaluation}

{\al 
TRAINING details: 10000 epochs, learning rate of 0.0005, batch size 16, euclidean loss for the graph and MSE for the force loss. Trained over 12 samples (x2) and tested on 3 samples (x2).
In this section we want to evaluate the proposed model by answering the following questions:
{\red probably all the evaluation should be done over the entire test set }
\begin{itemize}
    \item OK what is the effect of conditioning a GNN on force feedbacks? And to include the prediction of the forces to model the force dynamics?
    \item OK what is the quality of the graph prediction with respect to a standard GNN: short horizon, medium horizon, long horizon {\red (mean of all starting point) plus some images with different starting point}.
    \item OK what is the effect of the context gathered during the offline interaction?
    \item OK what is the quality of the prediction of the force wrt an standart MLP and a Linear prediction? {\red define what we mean with linear prediction. Show long, short, medium horizon  from different starting points and for different sample? O same samples? Probably very elastic and very rigid samples wuold be better.}
    \item OK what is the effect of the different conditioning on the force prediction?
    \item is the graph helping on predicting the force as it has the chance to distinguish between different intervals?
    \item does multiple propagation layers improve?
    \item what are the capabilities of these models to generalize over unseen actions? {\red for this part I would pick just one type of rollout and evaluate all the datasets on different action prediction, like 2 or 4}
    \item what is the effect of different datasets, is the mixed one imporving the results?
\end{itemize}
}

\subsection{Graph prediction}
{\al 
Evaluation on different datasets and different horizon length. The rollout is computed averaging the loss computed for each possible starting point of the rollout of each test sample. To understand the prediction capabilities of out model we compare it with a standard GNN that does not predict the Force feedback.

\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Steps& GNN & \multicolumn{2}{c}{GNN df1} & \multicolumn{2}{c}{GNN df4} \\
        \cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.         & - & no C & C  & no C & C  \\ \midrule
         1  &  \textbf{0.0146}  & 0.0265 &0.0363 &0.0216 & 0.0195 \\
         3  &  0.164 & 0.146& 0.128 & \textbf{0.121} & 0.131 \\
         5  & 0.629 & 0.607& 0.610 & 0.604 & \textbf{0.455} \\
         7  & 1.412   &  1.581&  1.549& 1.333 &   \textbf{1.135}\\ \bottomrule
    \end{tabular}
    \caption{Graph prediction error rollout 5 compared VS standard GNN}
    \label{tab:GNN_comp.}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Steps& GNN & \multicolumn{2}{c}{GNN df1} & \multicolumn{2}{c}{GNN df4} \\
        \cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.         & - & no C & C  & no C & C  \\ \midrule
          1  &  \textbf{0.0235}  & 0.0581 &0.0871 &0.0433 &0.0384\\
          3  &  0.757 & 0.671& \textbf{0.543} & 0.568 & 0.597 \\
          5  & 2.70 & 2.86& 2.67 & 2.34 & \textbf{1.99} \\ 
          7  & 5.634  & 6.574 & 7.592 & 5.595 &  \textbf{4.911} \\ \bottomrule
    \end{tabular}
    \caption{Graph prediction error rollout 10 compared VS standard GNN}
    \label{tab:GNN_comp.}
\end{table}



\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Steps& GNN & \multicolumn{2}{c}{GNN df1} & \multicolumn{2}{c}{GNN df4} \\
        \cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.         & - & no C & C  & no C & C  \\ \midrule
         1   &  \textbf{0.0273}  & 0.140 &0.227&0.0810  & 0.0771 \\
        3 &  3.34 & 3.33& \textbf{2.29} &2.69 & 2.79 \\
         5  & 10.9 & 19.1& 8.80 & 11.8 & \textbf{7.19} \\ 
         7  &  19.77 & 27.48 & 39.94 & 21.47 &   \textbf{18.55}\\ \bottomrule
    \end{tabular}
    \caption{Graph prediction error rollout 30 compared VS standard GNN}
    \label{tab:GNN_comp.}
\end{table}



The results on the step = 1 are not very good, but probably the task is too easy and there are no big differences between each consecutive image. This might be even destructive on the mixed dataset. To understand it's effect we trained the models on two different mixed dataset, one were the 1 step action is included and the other one where we removed it. Waiting for the results.
{\red comparison between performances of mixed dataset where 1 step is included vs 1 step not included.}

..............

Once evaluated the performances, is interesting to understand the role of including on the model the force dynamics. To evaluate these we chose to make the comparison on the rollout length = 10 and all the dataset. We focus just on one type of conditioning that is the one with multiple delta force as conditioning and prediction.


\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Steps&  \multicolumn{3}{c}{GNN no F model} & \multicolumn{2}{c}{GNN F model} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-6}
          pred.         & - & no C & C  & no C & C  \\ \midrule
         1   &  0.0235  &  \textbf{0.0182} &0.0238 &0.0433  & 0.0384 \\
        3 &  0.757 & 0.676 & 0.652 & \textbf{0.568}& 0.597 \\
         5  & 2.70 & 2.68 & 2.19 & 2.67 & \textbf{1.99} \\ 
         7  & 5.634  &  5.378 & 5.232 & 5.595 &  \textbf{4.911} \\ \bottomrule
    \end{tabular}
    \caption{Graph prediction error rollout 10. Effect of the types of conditioning and on the modelling of the force dynamics.}
    \label{tab:GNN_dynamic_force_comparison}
\end{table}

As can be seen from the table \ref{tab:GNN_dynamic_force_comparison}, including in the model the force dynamics is beneficial for the graph prediction imporving the model performances like suggested in \cite{murthy2020gradsim}.

Visualization of the predictions of the models on the 10 steps rollout starting from 3 different positions: initial, early middle, late middle. The comparison is between the baseline and the best model that is the one that models the force profile based on test textile 5.


\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp0_tx5_fig10.png}
         \caption{Starting position 0}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp5_tx5_fig10.png}
         \caption{Starting position 5}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp10_tx5_fig10.png}
         \caption{Starting position 10}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Rollout for dataset 3}
        \label{fig:graph_prediction_d3 }
\end{figure}




\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw5_rl10_sp0_tx5_fig10.png}
         \caption{Starting position 0}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw5_rl10_sp5_tx5_fig10.png}
         \caption{Starting position 5}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw5_rl10_sp10_tx5_fig10.png}
         \caption{Starting position 10}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Rollout for dataset 5}
        \label{fig:graph_prediction_d5 }
\end{figure}





\subsection{Force Prediction}

In this section we want to evaluate the prediction capabilities of our model. To do it we compare it with a standard MLP with the same architecture but without the graph information and without the propagation steps of the GNN.


\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Steps& Linear & \multicolumn{2}{c}{MLP df1} & \multicolumn{2}{c}{GNN df1} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.   & -      & no C & C  & no C & C\\ \midrule
         1   &0.435 &   0.395 & 0.276 &0.454 &  \textbf{0.254} \\
         3  & 2.835 &  1.898 &  \textbf{0.435} & 0.939 & 0.639\\
         5  & 7.461 & 4.617&  \textbf{0.752} &2.049 & 1.451 \\
         7  & 12.08 & 7.469  &  \textbf{0.668} & 4.995 & 0.821  \\ \bottomrule
         \toprule
        Steps& Linear &  \multicolumn{2}{c}{MLP df4} & \multicolumn{2}{c}{GNN df4} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.   & -      & no C & C  & no C & C\\ \midrule
         1   & 0.550&  0.275 &  \textbf{0.241} & 0.288 &0.286   \\
         3   & 0.548 &  0.286 &  \textbf{0.183} & 0.265 &  0.203 \\
         5   & 0.622 & 0.345 &  \textbf{0.148} & 0.272 & 0.224 \\
         7   &0.803 & 0.298  &  \textbf{0.123}  & 0.498  &  0.217 \\ \bottomrule
    \end{tabular}
    \caption{Force prediction error rollout 5. Comparison MLP VS GNN}
    \label{tab:GNN_comp.}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Steps&  Linear & \multicolumn{2}{c}{MLP df1} & \multicolumn{2}{c}{GNN df1} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.   & -      & no C & C  & no C & C\\ \midrule
         1   & 0.889 &  0.810  &  \textbf{0.307} &  0.399& 0.182 \\
         3   & 6.603 &  4.727 &  \textbf{0.443} & 2.438 & 0.632 \\
         5   & 14.06& 10.038 &  \textbf{0.768} & 5.862 & 1.804 \\
         7   & 12.81 &  10.91 &   \textbf{0.701} & 12.74 & 1.896 \\ \bottomrule
         \toprule
        Steps& Linear &  \multicolumn{2}{c}{MLP df4} & \multicolumn{2}{c}{GNN df4} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.   & -      & no C & C  & no C & C\\ \midrule
         1   & 0.541 & 0.319 &  \textbf{0.200} & 0.320&  0.205\\
         3  &  0.714 & 0.417 &  \textbf{0.138} & 0.378 & 0.157\\
         5  & 0.908  &  0.571 &  \textbf{0.110} & 0.469 &  0.240 \\
         7  &0.755 &  0.292 &  \textbf{0.090}  &  0.511 &   0.235\\ \bottomrule
    \end{tabular}
    \caption{Force prediction error rollout 10. Comparison MLP VS GNN}
    \label{tab:GNN_comp.}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Steps& Linear &  \multicolumn{2}{c}{MLP df1} & \multicolumn{2}{c}{GNN df1} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.   & -      & no C & C  & no C & C\\ \midrule
         1  & 0.186 &  0.146  & 0.129 & 0.152&  \textbf{0.024} \\
         3  & 1.264 &   0.959 &  \textbf{0.160} & 3.695 & 0.166 \\
         5  & 2.852 & 3.021 &  \textbf{0.702} & 6.387 & 3.032  \\
         7  & 4.278 & 3.393 &  \textbf{0.345 } & 1.777 & 5.151  \\ \bottomrule
         \toprule
        Steps& Linear &  \multicolumn{2}{c}{MLP df4} & \multicolumn{2}{c}{GNN df4} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-4}\cmidrule(lr){5-6}
          pred.   & -      & no C & C  & no C & C\\ \midrule
         1   & 0.136 &   0.101 &  \textbf{0.067} &0.120 &  0.072\\
         3  & 0.148 &  0.100 &   \textbf{0.038} & 0.199 & 0.070 \\
         5  &  0.199 &  0.124 &  \textbf{0.046 }& 0.418 & 0.743 \\
         7  & 0.236 & 0.067  &  \textbf{0.030} &  0.463 &   0.410 \\ \bottomrule
    \end{tabular}
    \caption{Force prediction error rollout 30. Comparison MLP VS GNN}
    \label{tab:GNN_comp.}
\end{table}


General comments:
\begin{itemize}
    \item The accuracy increases when there are multiple parameters given to the model to infer the force after the applied action
    \item Conditioning on the profile of the sample improves the prediction performance
    \item MLP generally outperforms our model but not by far
\end{itemize}
{\red In the final version of the paper we could use just the results of the best model and perform an ablation study of how the performance decrease when the conditioning is made on a smaller number of deltas. This is related to the fact that the force profile is not linear therefore it requires more than one conditioning parameter to have an accurate prediction of the force profile.}

Visualization of the results. We want to compare the predictions of the force rollout like we did for the graphs. In this case the baselines are the MLP prediction and the identity prediction {\red missing the mean of the dataset, but what we can do is to evauate different samples like elastic and rigid one}
We focus on just the comparison of the prediction of multiple forces {\red need to find a better way to describe this model} for each step as it's the best way to condition the prediction model. As we did for the graph, we evaluate the 10 steps rollout statring from three different initial position of the execution with three different testing samples. 


\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp0_tx1_force_comparison.png}
         \caption{Starting position 0, textile 1.}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp0_tx3_force_comparison.png}
         \caption{Starting position 0, textile 3.}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp0_tx5_force_comparison.png}
         \caption{Starting position 0, textile 5.}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Rollout for dataset 3}
        \label{fig:graph_prediction_d5 }
\end{figure}






\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp10_tx1_force_comparison.png}
         \caption{Starting position 10, textile 1.}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp10_tx3_force_comparison.png}
         \caption{Starting position 10, textile 3.}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/rw3_rl10_sp10_tx5_force_comparison.png}
         \caption{Starting position 10, textile 5.}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Rollout for dataset 3}
        \label{fig:graph_prediction_d5 }
\end{figure}


\subsection{Ablation: multiple propagation layers}

Having multiple propagation layers should help as the elastic model can be represented by a non-linear function composed by many layers. The challenge here might be that we don't have enough data to train the models. {\red should be tested with simulated data}. In what follows, we investigate the effect of having multiple propagation layers for the dataset 3. It can be seen that it help the graph prediction. For what concern the forces instead

\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Rollout & GNN & \multicolumn{2}{c}{GNN df1} & \multicolumn{2}{c}{GNN df4} \\
        \cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
         steps         & - & no C & C  & no C & C  \\ \midrule
         5   & 0.119  &  0.099 &0.087 &0.084 & \textbf{0.067} \\
         10  & 0.609 &0.442 & 0.446 & 0.409 & \textbf{0.361} \\
         30  &   2.828 &2.212 & 2.092 & 1.835 &\textbf{1.576}  \\ \bottomrule
    \end{tabular}
    \caption{Graph prediction error of GNN with multiple propagation layers for dataset 3.}
    \label{tab:GNN_comp.}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{lccccl}\toprule
        Rollout & GNN & \multicolumn{2}{c}{GNN df1} & \multicolumn{2}{c}{GNN df4} \\
        \cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
         steps         & - & no C & C  & no C & C  \\ \midrule
         5   & 0.164  &  0.146 &0.128 &\textbf{0.121} & 0.131 \\
         10  & 0.757 &0.671 & \textbf{0.543} & 0.568& 0.597 \\
         30  &  3.340 &3.330 &\textbf{ 2.290} & 2.690 &2.790  \\ \bottomrule
    \end{tabular}
    \caption{Graph prediction error of GNN with SINGLE propagation layers for dataset 3.}
    \label{tab:GNN_comp.}
\end{table}



\begin{table}[h]
    \centering
    \begin{tabular}{lcccl}\toprule
        Rollout&   \multicolumn{2}{c}{GNN df1 - S} & \multicolumn{2}{c}{GNN df4 - S} \\
         \cmidrule(lr){2-3}\cmidrule(lr){4-5}
          steps        & S & M  & S & M\\ \midrule
         5  &  0.639 &  2.710   & \textbf{0.203} & 0.354 \\
         10 &  0.632 &  0.316   & \textbf{0.157} &0.453 \\
         30 &   0.166  & 0.120  &\textbf{ 0.070} &   0.273\\ \bottomrule
        
    \end{tabular}
    \caption{Force prediction error rollout 30. Comparison MLP VS GNN}
    \label{tab:GNN_comp.}
\end{table}





}

% Second version of table, with booktabs.
% \begin{tabular}{lcccccl}\toprule
% Steps& \multicolumn{2}{c}{GNN} & \multicolumn{2}{c}{GNN df} & \multicolumn{2}{c}{GNN df+t} 
% \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%   pred.         & not L  & L & not L   & L  & not L & L\\\midrule
%  1   & 4.24 & 4.23  & 4.29 &4.19 &4.19  & \textbf{4.18} \\
% 3 & 6.73 & 6.39 & 6.36& \textbf{6.11} & 6.80 & 6.13  \\
%  5  & 10.7 & 10.23 & 9.38& \textbf{8.11} & 8.15 & 8.70 \\\bottomrule
%  \caption{Graph prediction error x10-3}
%  \label{tab:GNN_comp.}
% \end{tabular}

\subsection{Simulation Application - if provided by Yufei}



\subsection{Real World Application}
Here the main idea is to apply our learned model in a simplified version of assistive dressing scenario.

 \begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{images/skull_before.jpeg}
   \includegraphics[width=\linewidth]{images/skull_after.jpeg}
  \caption{Real world application with a dead body}
   \label{fig:real_world}
\end{figure}

% \subsection{Model Parameters}


